Automated Modular Verification for Race-Free Channels with Implicit and Explicit Synchronization

Ensuring the correctness of software for communication centric programs is important but challenging. Previous approaches, based on session types, have been intensively investigated over the past decade. They provide a concise way to express protocol specifications and a lightweight approach for checking their implementation. Current solutions are based on only implicit synchronization, and are based on the less precise types rather than logical formulae. In this paper, we propose a more expressive session logic to capture multiparty protocols. By using two kinds of ordering constraints, namely "happens-before" <HB and "communicates-before" <CB, we show how to ensure from first principle race-freedom over common channels. Our approach refines each specification with both assumptions and proof obligations to ensure compliance to some global protocol. Each specification is then projected for each party and then each channel, to allow cooperative proving through localized automated verification. Our primary goal in automated verification is to ensure race-freedom and communication-safety, but the approach is extensible for deadlock-freedom as well. We shall also describe how modular protocols can be captured and handled by our approach.

==> disjunct.tex <==
\subsection{Well-Formed Disjunction}
General disjunctions over multiple parties pose some
challenges, as they need to be 
synchronized across all the
affected parties. That is decision taken 
in choosing a disjunct to execute (or follow)
would have to be communicated to all parties involved in the
disjunction. This is non-trivial and would require extra
synchronization across multiple parties.
Furthermore, the
orderings that arise from a disjunctive specification
would have to be classified as {\em maybe}-orderings
rather than {\em must}-orderings. In this paper, we
propose a simpler alternative which places a
{\em well-formed} restriction on disjunction.

Consider a disjunctive specification:
{\footnotesize\[
  \code{((\atransmit{S}{R}{v\,{\cdot}\,\fmsg_1}{\chanvar}{\atid_1};G_1)
    \vee \cdots \vee
    (\atransmit{S}{R}{v\,{\cdot}\,\fmsg_m}{\chanvar}{\atid_m};G_m)  )}
\] }\vspace*{-2mm}
%% \begin{verbatim}
%%  (S->R:c<v;Q_1>;C1 \/ ..\/ S->R:c<v;Q_m>;C_m)
%% \end{verbatim}

For it to be well-formed, we must have
a common sender
\code{S} and a common receiver \code{R} 
at the start of this disjunction. %% Conventioally,
The common sender is said to be making an {\em internal choice}, while
the common receiver relies on an {\em external choice}.
Moreover, the resource transmitted \code{\fmsg_1{\cdots}\fmsg_m} 
must be disjoint, namely:
%
{\footnotesize \[
\code{\forall i,j \in \{1..m\}{\cdot} i{\neq}j \implies
  \fmsg_i{\wedge}\fmsg_j {=}\false } \] }

The reason for disjointness is to allow %% sufficient
static information to determine
%% that would allow determination
%% on 
which disjunctive path(s) have been taken.
Another condition we place on well-formed disjunction
is that the follow-up formulae \code{G_1{\cdots}G_m}
are restricted to transmissions between
the two common parties \code{S} and \code{R}.
While this may appear restrictive, the only parties
that are able to statically determine which disjunctive
path is chosen are just the two parties %% who
%% are []
making internal and external choices, respectively.
Moreover, the presence of external parties would
lead to {\em maybe}-orderings since some path may have
the orderings, while others would not.
In contrast, the common sender/receiver pair,
namely \code{S} and \code{R} themselves, would be
unambiguously captured in all the disjunctive 
branches. Thus, all orderings for these two
parties beyond the disjunction would thus hold
transitively on all branches. As a consequence, we can
support {\em must}-ordering
information using just %% ordering
constraints
from one of the branches.
As an example, consider the events from
the common sender, \code{S}, as follows:

\centerline{\footnotesize
\code{\betw{S^1}~;~(\betw{S^2} \vee \betw{S^3})~;~\betw{S^4}}
}

Though events \code{S^2} and \code{S^3} are present only
in the respective disjunctions, we could utilize
the ordering constraints, such as 
\code{\lthb{S^1}{S^2}} and \code{\lthb{S^2}{S^4}},
as {\em must} \code{\precx{HB}}-ordering.
Within the branch itself, orderings such as
\code{\lthb{S^1}{S^2}} are indeed must-ordering
since they must occur within the branch to support
reasoning within the corresponding conditional
code of \code{S}. 
Furthermore, beyond the disjunct itself,
 we could conclude 
%% that
its transitive outcome, namely \code{\lthb{S^1}{S^4}}, 
using information from only one branch %% is sufficient
since well-formedness requires the common
sender/receiver to be present in all
branches and moreover exclusively so. That is we 
can safely assume:

\centerline{\footnotesize
\code{(\lthb{S^1}{S^2}{\wedge}\lthb{S^2}{S^4}
  ~\vee \lthb{S^1}{S^3}{\wedge}\lthb{S^3}{S^4}) ~\implies~ \lthb{S^1}{S^4}}
}

With our well-formedness restriction on all
disjunctive formula, we could safely consider all
global orderings as a single conjunctive formula.
That is, for our example, it
is safe to strengthen our program state 
for global orderings to:

\centerline{\footnotesize
\code{(\lthb{S^1}{S^2}{\wedge}\lthb{S^2}{S^4}
  ~\wedge \lthb{S^1}{S^3}{\wedge}\lthb{S^3}{S^4})}
}

While this strengthening is unsound for normal disjunction,
we can show that it remains sound under our
well-formedness restriction and where all events are
uniquely labelled.

%% \input{partial-disj}


==> fig1.tex <==
\begin{figure}
\centering
\captionsetup[subfigure]{labelformat=empty,farskip=1pt,captionskip=1pt}  
\subfloat[][]
{\footnotesize
  $ 
  \arraycolsep=1pt
  \begin{array}{llll}
 \textit{Single ~ transmission}~ & \code{\terminal}& {~ ::=}& \quad \code{\atransmit{S}{R}{v\,{\cdot}\,\fmsg}{\chanvar}{\atid}}\\
  \textit{Global~protocol}& \code{\prot% (\rolevar^*)
                   } &{~ ::=} &\code{~~~ \terminal}\\
  %% Delegation &&&   ~|~ \code{\delegate{A}{B}{\prot}} \\
  %% Predicate~ instantiation &&& ~|~ \code{\view{p}{R^*,v^*}}\\
  %% Explicit~ sync && ~|~ \gdown{R}{\chanvar}{id} ~|~ \gawait{R}{\chanvar}{id}  \\
    %% ~|~ \zeta
  \textit{Concurrency} &&& ~|~ \code{\prot\,{\useq}\,\prot} \\
  \textit{Choice} &&& ~|~ \code{\prot\,{\vee}\,\prot } \\
  %% Strict~ %% 
  \textit{Sequencing}
  &&& ~|~ \code{\prot\,{\gseq{}}\,\prot} \\
  \textit{Guard} &&& ~|~ \code{\guard{\racefreeas}} \\
  \textit{Assumption} &&& ~|~ \code{\assume{\racefreeas}} \\
  \textit{Inaction} &&&   ~|~ {\emp}
  \end{array}
  $}%\\
% \subfloat[][]{\footnotesize
%   $
% \arraycolsep=1pt
% \begin{array}{rcl}
%   \code{(\prot_1{\seq} \prot_2){\seq}\prot_3} &{=}& \code{\prot_1{\seq}(\prot_2{\seq}\prot_3) }
% \\
%   \code{(\prot_1{\star}\prot_2){\star}\prot_3} &{=}& \code{\prot_1{\star}(\prot_2{\star}\prot_3) }
% \\
% \code{(\prot_1~\vee~\prot_2)~\vee~\prot_3} &{=}& \code{\prot_1~\vee~(\prot_2~\vee~\prot_3) }
% \\
% \code{\prot_1~\star~\prot_2} &{=}& \code{\prot_2~\star~\prot_1}
% \\
% \code{\prot_1~\vee~\prot_2} &{=}& \code{\prot_2~\vee~\prot_1}
% \\
% \code{\prot ~\star~\emp} &{=}& \code{\prot}
% \\
% \code{\emp~\seq~\prot } &{=}& \code{\prot}
% \\

% \end{array}
% $
% }
\subfloat[][]{\footnotesize
  $ 
  \arraycolsep=3pt
  \begin{array}{llll}
    \code{\text{\emph{(Parties)}}~ S,R \in \roletyp} \qquad
    \code{\text{\emph{(Channels)}}~\chanvar \in \chantyp } \qquad
    \code{\text{\emph{(Labels)}}~{\atid} \in \labeltyp } \qquad
    \code{\text{\emph{(Messages)}}~v\,{\cdot}\,\fmsg ~\text{~~~s.t.~}~ ~v \in \Var }
  \end{array}
  $
}
\vspace*{-2mm}
\hrule
\vspace*{-3mm}
\caption{\sessionlogic~ I: A Logic for Global Protocol Specification}
\label{fig.global_syntax}
\vspace*{-3mm}
\end{figure}


==> fig_safe_transmission.tex <==
\def\fidelity{
\begin{figure}
% \arraycolsep=1pt
\begin{flushleft}
\captionsetup[subfigure]{labelformat=empty,farskip=-4pt,captionskip=0pt}  
\subfloat[][]
{$% \footnotesize
  \begin{array}{ll}
    \code{\safefid{\lchanvar}{\rolevar}{(\atransmit{S}{R}{v{\cdot}\fmsg}{\lchanvar_0}{\atid}{\seq}\prottail)}} 
    &\code{\defeq~} 
      \code{(\SAFE,~{v{\cdot}\fmsg},~\atransmit{\HOLE}{R}{v{\cdot}\fmsg}{\lchanvar_0}{\atid}{\seq}\prottail)} 
      \text{~when~} 
      \code{\lchanvar_0 {=} \lchanvar ~\wedge~S {=} \rolevar}\\
    
    \code{\safefid{\lchanvar}{\rolevar}{(\atransmit{S}{R}{v{\cdot}\fmsg}{\lchanvar_0}{\atid}{\seq}\prottail)}} 
    &\code{\defeq~} 
      \code{(\SAFE,~{v{\cdot}\fmsg},~\atransmit{S}{\HOLE}{v{\cdot}\fmsg}{\lchanvar_0}{\atid}{\seq}\prottail)} 
      \text{~when~} 
      \code{\lchanvar_0 {=} \lchanvar ~\wedge~R{=} \rolevar }\\

    \code{\safefid{\lchanvar}{\rolevar}{(\atransmit{S}{R}{v{\cdot}\fmsg}{\lchanvar_0}{\atid}{\seq}\prottail)}}
    &\code{\defeq~}
      \code{(\ANS,~\msgvar,~\atransmit{S}{R}{v{\cdot}\fmsg}{\lchanvar_0}{\atid}\seq\protres)}
      \text{~when~} 
      \code{\rolevar {\notin} \{S,~R\} ~\wedge~ \lchanvar{\neq}\lchanvar_0
      }\\
    \multicolumn{2}{r}{\code{~\wedge~ (\ANS,~\msgvar,~\protres) {=} \safefid{\lchanvar}{\rolevar}{\prottail} }}\\

    \code{\safefid{\lchanvar}{\rolevar}{(\prot_1 \vee \prot_2){\seq}\prottail}}
    &\code{\defeq~}
    \code{(\ANS,~\msgvar,~(\protres \vee \prot_2) \seq\prottail)}
    \text{~when~} 
    \code{(\ANS,~\msgvar,~\protres) {=}
      \safefid{\lchanvar}{\rolevar}{\prot_1}} \\
    \multicolumn{2}{r}{ \code{~\wedge~ (\FAIL,~{\_},~{\_}) {=} \safefid{\lchanvar}{\rolevar}{\prot_2} }}\\
&   \text{~or~}
    \code{(\ANS,~\msgvar,~(\prot_1 \vee \protres) \seq\prottail)}
    \text{~when~} 
    \code{(\FAIL,~{\_},~{\_}) {=}
  \safefid{\lchanvar}{\rolevar}{\prot_1} }\\
    \multicolumn{2}{r}{\code{~\wedge~
    (\ANS,~\msgvar,~\protres) {=}
    \safefid{\lchanvar}{\rolevar}{\prot_2}}}\\
    
    \code{\safefid{\lchanvar}{\rolevar}{(\prot_1 \useq \prot_2){\seq}\prottail}}
    &\code{\defeq~}
      \code{(\ANS,~\msgvar,~(\protres \useq \prot_2) \seq\prottail)}
      \text{~when~} 
      \code{(\ANS,~\msgvar,~\protres) {=}
      \safefid{\lchanvar}{\rolevar}{\prot_1}}\\
    \multicolumn{2}{r}{\code{~\wedge~ (\FAIL,~{\_},~{\_}) {=} \safefid{\lchanvar}{\rolevar}{\prot_2} }}\\
    &   \text{~or~}
      \code{(\ANS,~\msgvar,~(\prot_1 \useq \protres) \seq\prottail)}
      \text{~when~} 
      \code{  (\FAIL,~{\_},~{\_}) {=}
      \safefid{\lchanvar}{\rolevar}{\prot_1}}\\
      \multicolumn{2}{r}{\code{~\wedge~ (\ANS,~\msgvar,~\protres) {=} \safefid{\lchanvar}{\rolevar}{\prot_2}}}
  \end{array}
  $} \hfill \\
% \vspace*{5mm}
\end{flushleft}
% \hspace*{-30mm}
\vspace*{-3mm}
\hrule
\vspace*{3mm}
\caption{Safety Check: Protocol Conformance}\label{fig.semantics.fidelity}
% \vspace*{-3mm}
\end{figure}
}

\def\racefreecheck{
\begin{figure}
  % \arraycolsep=1pt
  \begin{flushleft}
\captionsetup[subfigure]{labelformat=empty,farskip=-4pt,captionskip=0pt}  
\subfloat[][]
{$% \footnotesize
  \begin{array}{ll}
    \code{\safesnd{(\atransmit{S}{R}{v{\cdot}\fmsg}{}{\atid}{\seq}\cprojtail)}{\rolevar}{\msgvar}{\sigma}} &\code{\defeq~} 
    \code{\SAFE } % ,{v{\cdot}\fmsg} 
    \text{~when~}  \code{\rolevar {=} S
}\\
    \code{\safesnd{(\atransmit{\HOLE}{R}{v{\cdot}\fmsg}{}{\atid}{\seq}\cprojtail)}{\rolevar}{\msgvar}{\sigma}}
    &\code{\defeq~}
     \code{\safesnd{\cprojtail}{\rolevar}{\msgvar}{\sigma}}
     \text{~when~} 
     \code{\rolevar {\neq} R    }\\
    \code{\safesnd{((\cproj_1 {\vee} \cproj_2){\seq}\cprojtail)}{\rolevar}{{\msgvar}}{\sigma}}
    &\code{\defeq~}
      \code{ \safesnd{\cproj_1}{\rolevar}{\msgvar}{\sigma} }
      \text{~when~} 
      \code{\FAIL {=} \safesnd{\cproj_2}{\rolevar}{\msgvar}{\sigma}}\\
    & \text{\quad ~or~~  }
      \code{\safesnd{\cproj_2}{\rolevar}{\msgvar}{\sigma}}
      \text{~when~} 
      \code{\FAIL {=} \safesnd{\cproj_1}{\rolevar}{\msgvar}{\sigma}}    
%    % \code{\qquad|~\FAIL,~\cproj} &
    % \multicolumn{2}{l}{\code{otherwise}}  
  \end{array}
$}% \hspace{10mm}
\hfill 
% \vspace*{5mm}
\subfloat[][]
{$% \footnotesize
  \begin{array}{ll}
    \code{\safercv{(\atransmit{\HOLE}{R}{v{\cdot}\fmsg}{}{\atid}{\seq}\cprojtail)}{\rolevar}} &\code{\defeq~} 
    \code{\SAFE} 
    \text{~when~} 
    \code{\rolevar {=} R}\\
    \code{\safercv{(\atransmit{S}{R}{v{\cdot}\fmsg}{}{\atid}{\seq}\cprojtail)}{\rolevar}} &\code{\defeq~} 
    \code{\BLOCK}
    \text{~when~} 
    \code{\rolevar {=} R}\\
    \code{\safercv{(\atransmit{\HOLE}{\HOLE}{\_}{}{\atid}{\seq}\cprojtail)}{\rolevar}}
    &\code{\defeq~}
    \code{\safercv{\cprojtail}{\rolevar}}\\
    \code{\safercv{((\cproj_1 {\vee} \cproj_2){\seq}\cprojtail)}{\rolevar}}
    &\code{\defeq~}
    \code{\safercv{\cproj_1}{\rolevar} }
      \text{~when~} 
    \code{\FAIL {=} \safercv{\cproj_2}{\rolevar}}\\
    & \text{\quad ~or~~  }
    \code{\safercv{\cproj_2}{\rolevar} }
    \text{~when~} 
    \code{\FAIL {=} \safercv{\cproj_1}{\rolevar} }
    \\
%&
  \end{array}
  $}\hfill
\end{flushleft}
% \vspace*{5mm}
\vspace*{-3mm}
\hrule
\vspace*{3mm}
\caption{Safety Checks: Race-free}\label{fig.safe_transmission}
% \vspace*{-3mm}
\end{figure}
}

\def\figsafeemp{
\begin{figure}
  % \arraycolsep=1pt
\begin{center}
\captionsetup[subfigure]{labelformat=empty,farskip=-4pt,captionskip=0pt}  
\subfloat[][]
{$% \footnotesize
  \begin{array}{ll}
    \code{\safeemp{\rolevar^*}{(\atransmit{S}{R}{\_}{}{\atid})}} 
    &\code{\defeq~}
      \code{\forall \rolevar \in \rolevar^* \implies  \rolevar \notin \{S,R\}}\\
    \code{\safeemp{\rolevar^*}{\cproj_1 \seq \cproj_2}} 
    &\code{\defeq~}
      \code{\safeemp{\rolevar^*}{\cproj_1}  \wedge}
      \code{\safeemp{\rolevar^*}{\cproj_2}}\\
    \code{\safeemp{\rolevar^*}{\cproj_1 \vee \cproj_2}} 
    &\code{\defeq~}
      \code{\safeemp{\rolevar^*}{\cproj_1}  \vee}
      \code{\safeemp{\rolevar^*}{\cproj_2}}
  \end{array}
  $}\hfill
\end{center}
% \hspace*{-30mm}
% \vspace*{-3mm}
\hrule
\vspace*{3mm}
\caption{Safety Check: Leak-free}\label{fig.safe_empty}
% \vspace*{-3mm}
\end{figure}
}

==> fig_semantic_model.tex <==
% Proposed model:
% ============================
% Machine State  MS  ::= PS x CS

% Threads        PS  ::= idt -> TS

% Thread State   TS  ::= \heap x \stack x Prog
% Thread         TC  ::= TS x CS
% Configuration
% Thread Res     

% Channels State  CS ::= idc ->  Chan
% Channel       Chan ::= resource list 

% Thread id      idt ::= int


\begin{figure}%[H]
% % \vspace{-1em}
\begin{center}
\captionsetup[subfigure]{labelformat=empty,farskip=-5pt,captionskip=-15pt}  
\subfloat[][]
{$
  \begin{array}{llll}
    \textit{Machine~Config.} & \code{MC} &\!\!\!\code{::=}&
                                                             \code{\pstate ~ \times ~ \CH} \\
 \textit{Channels} & \code{\CH} &\!\!\!\code{::=}&
                       \code{\bringson{\echantyp}{(Val \cup Loc
                                                       % \times Type
                                                   )^*}}\\
 \textit{Program~State} &\code{\pstate} &\!\!\!\code{::=}&
                                                         \code{\bringson{\text{\idt}}{\LS}{}{}} \\
 \textit{Thread~State} &\code{ % {\itst}{\in}
                                \LS} &\!\!\!\code{::=}& \code{\btt{State} \times \btt{\Prog}} \\
 \textit{Local~State} &\code{ % {\tst}{\in}
                          {\btt{State}}}
                       &\!\!\!\code{::=}& \code{\btt{Stack} \times
                                          \btt{Heap} } \\
 \textit{Thread~Config.} &\code{\tconf} &\!\!\!\code{::=}& \code{\LS
                                                       ~\times~ \CH} \\
  \end{array}
$}\\
\subfloat[][]
{$
\begin{array}{lllll}
    \\
    \code{\PS{\in}\pstate} &
    \code{\TC{\in}\tconf} &
    \code{{\tst}{\in}{State}} &
    \code{{\ltst}{\in}{\LS}} &
    \code{\channel{\in}\CH} 
\end{array}
$}
\vspace*{3mm}
\hrule
\end{center}
% \vspace*{-3mm}
\caption{A Semantic Model of the Core Language }\label{fig.gen_semantic_model}
% \vspace*{-3mm}
\end{figure}



==> fig_spec_syntax.tex <==
%% ****************************************
%% ************ Spec Language *************
%% ****************************************
{\footnotesize
\begin{figure}%[htb!]
\begin{center}
{\footnotesize
\[\arraycolsep=1pt
\begin{array}{llll}
  \textit{Symbolic~ pred.} & \myit{pred} &::=& \view{p}{\self, v^*}~{\veq}~ \constr
  \mid \view{p}{\rolevar^*,v^*}~{\veq}~\prot
  \qquad

  \\
  \textit{Formula} &   \constr & ::=& \bigvee \St \qquad \qquad \St  ::= \exists ~ v^*{\cdot}\heap{\wedge}\pure 
  ~|~ \St * \St   
  \\
  %Resource
  \textit{Separation} & \heap &::=& \emp 
      ~|~ \mapview{v}{d}{v^*}
      ~|~ \view{p}{v^*}
      ~|~ \chani{v}{\rolevar}{\proj}
      ~|~ \heap \sep \heap
      ~|~ \hov
  \quad
  \\
  \textit{Pure} &\pure &::=& v:t 
  \mid \myit{b} \mid \myit{a} \mid 
                \phi {\wedge} \phi \mid \phi {\vee} \phi \mid \neg \phi  \\
  &&&
  \mid \exists v \cdot \phi \mid \forall v \cdot \phi \mid \ptr
  \\
  \textit{Pointer~ eq./diseq.}& \ptr &::=& v {=} v ~|~ v{=}\nil ~|~ v{\neq}v ~|~ v{\neq}\nil
  \\
  \textit{Boolean} & \myit{b} &::=& ~\!\true \mid \false %\mid v 
  \mid \myit{b} \!=\! \myit{b} \qquad
  \myit{a} ::= \!\a {=} \a
  \mid \a {\leq} \a
  \mid \hov{=}\St
  \\
  \textit{Presburger~ Arith.}~ & \a &::=&~ %\!\!\begin{array}[t]{l}
  \!k^{\int} \mid v \mid k^{\int}{\times}\a
  \mid \a \!+\! \a 
  \mid - \a   \\
  &&& \\
  %\hsbody{
  &\text{where} &&  k^{\int} \text{~: ~integer~constant;}~ v \text{~:~ first~ order~ variable};\\
  &&& \hovars \text{~:~ second-order~ variable};~\rolevar \text{~:~ session~ role}\\
  &&& d \text{~:~ name~ of~ a ~user-defined~ data~ structure}\\
  &&& \myit{L} \text{~:~local~protocol~(defined~in~Fig.~\ref{fig.proj_syntax})}
  %}
\end{array}
\]
}
\hrule
\vspace*{-3mm}
\caption{\sessionlogic~II: The (Program) Specification Language}
\label{fig.spec_syntax}
\vspace*{-3mm}
\end{center}
\end{figure}
}

==> mathbxpersonal.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% redefining some mathabx
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Setup the matha font (from mathabx.sty)
\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
  <5> <6> <7> <8> <9> <10> gen * matha
  <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
}{}

\DeclareSymbolFont{matha}{U}{matha}{m}{n}
\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * mathb
      <10.95> mathb10 <12> <14.4> <17.28> <20.74> <24.88> mathb12
      }{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}
      
\DeclareMathSymbol{\updownharpoons}        {3}{matha}{"EA}
\DeclareMathSymbol{\downupharpoons}        {3}{matha}{"EB}
\DeclareMathSymbol{\upupharpoons}          {3}{mathb}{"DA}
\DeclareMathSymbol{\downdownharpoons}      {3}{mathb}{"DB}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% redefining some mathabx
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> overview-long.tex <==
To capture a broad range of %% concurrent
communication patterns, we propose an
expressive logic for specification of global protocols
in \figref{fig.global_syntax}. 
%% \wnsay{move Fig 1 here ..}
This protocol uses
\code{\prot_1\,{\useq}\,\prot_2} for
%% non-deterministic communication
%% over
the concurrency of \code{\prot_1} and \code{\prot_2};
\code{\prot_1\,{\vee}\,\prot_2} for disjunctive choice between
either \code{\prot_1} and \code{\prot_2}
and finally \code{\prot_1\,{\gseqA{}}\,\prot_2} on
the implicit sequentialization of \code{\prot_1} before \code{\prot_2}
for either the same party or same channel communication.
Moreover, we express the message type of a transmission
\code{\atransmit{S}{R}{v\,{\cdot}\,\fmsg}{c}{\atid}}
by $\code{{v\,{\cdot}\,\fmsg}}$
which expects a message \code{v} on some resource
expressed in logical form \code{\fmsg} (whose definition is given  in Fig.~\ref{fig.spec_syntax})
transmitted over channel \code{c}.
As an example, \code{v\,{\cdot}\,\view{ll}{v,n}_{\frac{1}{2}}} would capture
the transmission of half fractional permission\footnote{Fractional permissions
are important for supporting concurrent programming.
Its use allows read access when a resource
is shared by multiple parties, but also
write access when a resource
later becomes exclusively owned.} of a linked list with
\code{n} elements
\code{\view{ll}{v,n}} rooted at \code{v}. 
Apart from messages in logical form, our %% proposed
session logic %% would also
captures %% non-deterministic
%% communication,
logical disjunction and 
%% also
can enforce explicit synchronization to
ensure communication safety.% \anay{should we remove the non-det reference?}

% \savespace
% \savespace

Apart from unique
transmission labels, we provide a specification refinement
that adds guards (of the form
\code{\guard{\racefreeas}}) and assumptions (of
the form \code{\assume{\racefreeas}}), as more precise
refinement of its global protocol. The former is used to
add assertions (or proof obligations), such as
explicit synchronization, into its
global protocol to ensure safe communications;
while the latter is used
to support flow of information 
across multiple parties to facilitate
local verification. To sketch the main
purpose of using these guards and assumptions,
we briefly introduce
elements of its information flow language later in this section.
Further details about \code{\racefreeas} are given in
\secref{sec.global.safety}.


These new specification
constructs are added automatically by our 
refinement procedure
to provide assumptions and proof obligations
%% which help
to ensure race-freedom in shared channels%%  and 
%% message safety in non-deterministic communications
.
Our refinement %% process
could %% be used to
add channel
information based on some expected communication patterns.
For example, if mailbox communication
style is preferred, each communication always directs its
message to the mailbox of its receiver. %% However,
If bi-directional channels of communication are preferred,
%% we would provide a 
a distinct channel is provided
for every pair of
parties that are in communication.
%% Other choices of communication patterns are also possible.
To support diversity, we %% ignore such a refinement and
assume channels are captured %% made 
explicitly in our
protocol specifications.
\wnnay{change R (Role) to P (Party)?}
\input{fig1.tex}

Our approach thus takes in a protocol
specified in an expressive logic, {\em refine} it,
then {\em project} it on a per party and per channel basis.
Once these are done, we can proceed to apply automated
verification on the entire program code using the
derived specs.
%% (i) specification logic for global protocol
%% (ii) spec refinement (with channels + identities)
%% (iii) role projection
%% (iv) automated verification

\hide{
 \input{example-overview}  %%%Florin's example%%%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%end-of-hide%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\wnnay{Florin : Can help typeset and improve above}
\wnnay{Florin: Can we have a diagrammatic overview of
our approach by a very simple example. Highlight (i) specification refinement (ii) spec projection (iii) automated verication}

%% \begin{verbatim}
%% Consider:

%%   A-1->C:k(t1); B-2->C:k(t2)

%% Refined spec:
%% -------------
%%  A-1->C:k;+(A^1);+(C^1);+(A^1 <_CB C^1); 
%%  B-2->C:k;+(B^2);+(C^2);+(C^1 <_HB C^2)
%%     ;+(B^2 >_CB C^2);-(1 <_HB 2)

%% Projecting by party gives:
%% --------------------------
%% !A;+(A^1);+(1 <_HB 2);

%% !B;+(B^2);-(1 <_HB 2)_{B};

%% ?C;+(C^1);?C;+(C^2);-(1 <_HB 2)_{C};

%% Projecting the shared specs:
%%  +(A^1 <_CB C^1);
%%  +(C^1 <_HB C^2);
%%  +(B^2 <_CB C^2);
%% \end{verbatim}

The automated verification is conducted against a general and expressive specification language based on Separation Logic \cite{reynolds2002separation,Chin:2012:AVS:2221987.2222283},  as shown in Fig.~\ref{fig.spec_syntax}, which supports the use of (inductive) predicates,  the specification of separation and numerical properties, as well as channel predicates. 

\input{fig_spec_syntax}

\subsection{Specification Refinement}

Let us use a well-known %% more substantive
example
to illustrate the key ideas of our approach.
Consider the multi-party
protocol from \cite{Honda:2008:MAS:1328897.1328472} where we use a
distinct channel as mailbox of each of the
three parties, namely seller \code{S},
first buyer \code{B_1} and the second collaborative buyer \code{B_2}.
%% .
%% but where we use
%% only two channels for three parties, namely
%% a seller (with its own mailbox \code{s})
%% and two buyers (with a common mailbox \code{b}) 
%% collaborating on
%% a shared purchase.
%% Refinement adding completed communication.
\hide{
\begin{verbatim}
B1->S:s(Order);
(S->B1:b(Price) * S->B2:b(Price));
(B1->B2:b(Amt));
(B2->S:s(No) \/ B2->S:s(Yes);B2->S:s(Addr))
\end{verbatim}
}

%% {\footnotesize
%%   \centering
%%   \arraycolsep=1pt
%%   \[
%%     \begin{array}{l}
%%       \code{
%%       \transmit{B_1}{S}{\omsg{v}{Order}}{s}~ \seq~} \\
%%       \code{(\transmit{S}{B_1}{\omsg{v}{Price}}{b} \useq
%%       \transmit{S}{B_2}{\omsg{v}{Price}}{b} )~ \seq~} \\
%%       \code{\transmit{B_1}{B_2}{\omsg{v}{Amt}}{b} ~\seq~ } \\
%%       \code{ (\transmit{B_2}{S}{\omsg{vR}{No}}{s}
%%       \vee
%%       ( \transmit{B_2}{S}{\omsg{v}{Yes}}{s} ~\seq~
%%       \transmit{B_2}{S}{\omsg{v}{Addr}}{s})
%%       )
%%       % (B2->S:s(No) \/ B2->S:s(Yes);B2->S:s(Addr))
%%       }
%%     \end{array}
%%   \]
%% }

%% \wnsay{example with deterministic 
%% concurrency supported by different channels}

{\footnotesize
  \centering
  \vspace*{-2mm}
  \arraycolsep=1pt
  \[\vspace*{-2mm}
    \begin{array}{l}
      \code{
      \transmit{B_1}{S}{\omsg{v}{Order}}{s}~ \seq~} \\
      \code{(\transmit{S}{B_1}{\omsg{v}{Price}}{b_1} \useq
      \transmit{S}{B_2}{\omsg{v}{Price}}{b_2} )~ \seq~} \\
      \code{\transmit{B_1}{B_2}{\omsg{v}{Amt}}{b_2} ~\seq~ } \\
      \code{ (\transmit{B_2}{S}{\omsg{vR}{No}}{s}
      \vee
      ( \transmit{B_2}{S}{\omsg{v}{Yes}}{s} ~\seq~
      \transmit{B_2}{S}{\omsg{v}{Addr}}{s})
      )
      % (B2->S:s(No) \/ B2->S:s(Yes);B2->S:s(Addr))
      }
    \end{array}
  \]
}

Note that \code{T} is a
short-hand for \code{\msg{v}{T(v)}} where
\code{T} is a type or predicate for 
some resource, such as
\code{Order}, \code{Price}, \code{Amt} or \code{Addr}.


For the above example, our refinement would add
information to signify the timely completion
of each communication completed using
\code{\assume{\atransmit{S}{R}{}{}{\atid}}}.  %% to capture 
%% each completed communication event.
This event itself
captures two locally observable events and a
globally observable ordering, as follows:
{\footnotesize
\[\vspace*{-2mm}
  \code{\assume{\atransmit{S}{R}{}{}{\atid}}} ~{\implies}~ \code{\assumeL{\event{S}{\atid}}{R}~{\wedge}~\assumeL{\event{R}{\atid}}{R}}~{\wedge}~\code{\assume{\ltcb{\event{S}{\atid}}{\event{R}{\atid}}}}
\]
}

\noindent
which indicates the occurrence of the send
and receive events
and the expected {\cb} %{\em communicated-before} 
ordering\footnote{Under race-free assumption,
%% We explain later why this 
\code{\precx{CB}} ordering is the same as \code{\precx{HB}}-ordering.},
denoted by \code{\precx{CB}}, for its
successfully completed communication.
The send and receive events are only observable locally.
For example, the completion of event \code{\assumeL{\event{\rolevar_1}{\atid}}{S}}
is only observable in party \code{\rolevar_1}, but not by other distinct
parties, such as \code{\rolevar_2}. Its occurrence in the global protocol
is thus location sensitive and can be used to
capture relative orderings within the same party.
However, the ordering
\code{\assume{\ltcb{\event{S}{\atid}}{\event{R}{\atid}}}} is globally observable
since it relates two parties and our assurance
that all send/receive events are uniquely labelled.
Later, we will see how immediately adjacent
\code{\precx{HB}} ordering information are generated from locally
observable events within each party, and how \code{\precx{HB}} orderings can
be transitively propagated from other
globally observable 
\code{\precx{CB}} and \code{\precx{HB}} orderings.

When common channels are involved, we
also use proof obligations of the form
\code{\guard{\lthb{\atid_1}{\atid_2}}} to denote two transmissions,
labelled \code{\atid_1} and \code{\atid_2}, that are expected to be sequentialized%% ;
%% and \code{\guard{\atid_3 {\useq} \atid_4}} for non-deterministic
%% communication
.
Assuming each transmission \code{\atid} be denoted
by \code{\atransmit{S_i}{R_i}{v{\cdot}\fmsg_i}{c}{\atid}}
with \code{\chanvar} as common channel,  
these proof obligations can be
further reduced, as follows:
{\footnotesize
\[\vspace*{-2mm}
\arraycolsep=1pt
\begin{array}{ll}
  \code{\guard{\lthb{\atid_1}{\atid_2}}}  &
  \code{{\equiv}~
  \guard{\lthb{\event{S}{\atid_1}_1}{\event{S}{\atid_2}_2}{\wedge}
  \lthb{\event{R}{\atid_1}_1}{\event{R}{\atid_2}_2}}} \\
 %%  \code{{\equiv}~
 %%  \guard{(\lthb{\event{S}{\atid_1}_1}{\event{S}{\atid_2}_2}{\wedge}
 %%  \lthb{\event{R}{\atid_1}_1}{\event{R}{\atid_2}_2})~\vee~(\lthb{\event{R}{\atid_1}_1}{\event{S}{\atid_2}_2}{\wedge}\lthb{\event{R}{\atid_1}_1}{\event{R}{\atid_2}_2}})} \\
 %% & \code{{\equiv}~
 %%  \guard{(\lthb{\event{S}{\atid_1}_1}{\event{S}{\atid_2}_2}{\wedge}
 %%  )~\vee~(\lthb{\event{R}{\atid_1}_1}{\event{S}{\atid_2}_2}{\wedge}\lthb{\event{R}{\atid_1}_1}{\event{R}{\atid_2}_2}})} 
  %% \code{\guard{\atid_3{\useq}\atid_4} } &
  %% \code{{\equiv}~ \guard{v{\cdot}\fmsg_3{\iff}v{\cdot}\fmsg_4}} \\
\end{array}
\]
}

The \code{\lthb{}{}} is overloaded for both transmissions
e.g. \code{\lthb{\atid_1}{\atid_2}} 
and events e.g. \code{\lthb{\event{P}{\atid_1}_1}{\event{P}{\atid_2}_2}}. 
In the definition of \code{\guard{\lthb{\atid_1}{\atid_2}}}, 
we used the weakest condition to ensure race-freedom over the
common channels for transmission \code{\atid_1} and \code{\atid_2}.
We ensure that the two senders are ordered by
\code{\guard{\lthb{\event{S}{\atid_1}_1}{\event{S}{\atid_2}_2}}}, and the two receivers are ordered by
\code{\guard{\lthb{\event{R}{\atid_1}_1}{\event{R}{\atid_2}_2}}}.
Our refined specification follows:
\hide{
From
the definition of \code{\guard{\lthb{\atid_1}{\atid_2}}}, there are
two different ways of ensuring
\code{\precx{HB}} ordering over two
sequential transmissions sharing the same channel.
The former condition is the minimum one required to ensure
race-freedom. The latter condition is a stronger condition
that implies the former, but needs only a
single synchronization object (that blocks at both \code{S_2} and
\code{R_2} waiting for \code{R_1} to be completed),
as opposed to two synchronization objects
(that blocks at \code{S_2} waiting for \code{S_1}
and at \code{R_2} waiting for \code{R_1}, respectively) in the former condition.}
\hide{The definition of \code{\guard{\atid_3{\useq}\atid_4}} ensures that messages over shared
channel in non-deterministic communication are logically equivalent to each other,
up to the abstraction level used to ensure protocol correctness.}
 %% -(l1 <_HB l2) to ensure that transmission
 %%               l1 occur before l2
 %%  = -(S_1 <_HB S_2 & R1 <_HB R_2 \/ R_1 <_HB S_2 & R_1 <_HB R_2)

 %% -(l1 * l2) to ensure that transmissions
 %%            l1 and l2 can occur non-deterministically

 %%  = -(v.C_3 <-> v.C_4)
 %%  +(R1-l1->R2:k(m)) to indicate that transmission
%% \hide{
%% \begin{verbatim}
%% B1-1->S:s(Order);+(B1-1->S)
%% (S-2->B1:b(Price);+(S-2->B1) * S-3->B2:b(Price);+(S-3->B2));
%% ;-(2 * 3);
%% (B1-4->B2:b(Amt));+(B1-4->B2);-(3 <_HB 4);-(2 <_HB 3);
%% (B2-5->S:s(No);+(B2-5->S);-(1<:_HB 5);
%%  \/ B2-6->S:s(Yes);+(B2-6->S);-(1<:_HB 6);
%%     B2-7->S:s(Addr);+(B2-7->S);-(6<:_HB 7);)
%% \end{verbatim}
%% }

%% \hide{
%% \wnsay{to change to b1 and b2}

%% {\footnotesize
%%   \centering
%%   \arraycolsep=1pt
%%   \[
%%     \begin{array}{l}
%%       \code{
%%       \atransmit{B_1}{S}{\omsg{v}{Order}}{s}{1}~ \seq~
%%       \blueord{\assume{\atransmit{B_1}{S}{}{}{1}}~ \seq}} \\
%%       \code{((\atransmit{S}{B_1}{\omsg{v}{Price}}{b}{2} ~\seq~
%%       \blueord{\assume{\atransmit{S}{B_1}{}{}{2}}})
%%       \useq
%%       (\atransmit{S}{B_2}{\omsg{v}{Price}}{b}{3} )~
%%       \seq~ \blueord{\assume{\atransmit{S}{B_2}{}{}{3}}}) } 
%%       %% \code{~\seq \blueord{\guard{2 \useq 3}}}
%%       \\
%%       \code{\atransmit{B_1}{B_2}{\omsg{v}{Amt}}{b}{4} ~\seq~
%%       \blueord{\assume{\atransmit{B_1}{B_2}{}{}{4}}} ~\seq~
%%       \blueord{\guard{\lthb{2}{4}} \seq \guard{\lthb{3}{4}}}   ~\seq} \\
%%       \code{ ((\atransmit{B_2}{S}{\omsg{v}{No}}{s}{5} ~\seq~
%%       \blueord{\assume{\atransmit{B_2}{S}{}{}{5}}} ~\seq~
%%       \blueord{\guard{\lthb{1}{5}}})
%%       ~\vee~ }\\
%%       \code{\;\,( \atransmit{B_2}{S}{\omsg{v}{Yes}}{s}{6} ~\seq~
%%       \blueord{\assume{\atransmit{B_2}{S}{}{}{6}}}  ~\seq~
%%       \blueord{\guard{\lthb{1}{6}}}
%%       }\\
%%       \code{\;\,\;\,
%%       \atransmit{B_2}{S}{\omsg{v}{Addr}}{s}{7} ~\seq~ 
%%       \blueord{\assume{\atransmit{B_2}{S}{}{}{7}}} ~\seq~
%%       \blueord{\guard{\lthb{6}{7}}}
%%       )
%%       ).
%%       % (B2->S:s(No) \/ B2->S:s(Yes);B2->S:s(Addr))
%%       }
%%     \end{array}
%%   \]
%% }
%% }

%% \wnsay{need to tidy below..}\scsay{is it okay now?}

{\footnotesize
  \centering
  \vspace*{-2mm}
  \arraycolsep=1pt
  \[\vspace*{-2mm}
     \code{\prot} \code{\defeq} 
     \begin{array}[t]{l}
      \code{
      \atransmit{B_1}{S}{\omsg{v}{Order}}{s}{1}~ \seq~
      \blueord{\assume{\atransmit{B_1}{S}{}{}{1}}~ \seq}} \\
      \code{((\atransmit{S}{B_1}{\omsg{v}{Price}}{b_1}{2} ~\seq~
      \blueord{\assume{\atransmit{S}{B_1}{}{}{2}}
      {\seq}\assume{{\lthb{\event{S}{1}}{\event{S}{2}}}}  
       {\seq}\assume{{\lthb{\event{B_1}{1}}{\event{B_1}{2}}}}  
       })}\\
     \code{~ \useq~
      (\atransmit{S}{B_2}{\omsg{v}{Price}}{b_2}{3} ~
      \seq~ \blueord{\assume{\atransmit{S}{B_2}{}{}{3}}
      {\seq}\assume{{\lthb{\event{S}{1}}{\event{S}{3}}}}  
      })) ~\seq~} 
      %% \code{~\seq \blueord{\guard{2 \useq 3}}}
      \\
     \code{\atransmit{B_1}{B_2}{\omsg{v}{Amt}}{b_2}{4} ~\seq~
      \blueord{\assume{\atransmit{B_1}{B_2}{}{}{4}}
      {\seq}\assume{{\lthb{\event{B_1}{2}}{\event{B_1}{4}}}}  
      {\seq}\assume{{\lthb{\event{B_2}{3}}{\event{B_2}{4}}}}  
      {\seq} \guard{\lthb{3}{4}}}   ~\seq} \\
     \code{ ((\atransmit{B_2}{S}{\omsg{v}{No}}{s}{5} ~\seq~
      \blueord{\assume{\atransmit{B_2}{S}{}{}{5}}
      {\seq}\assume{{\lthb{\event{B_2}{4}}{\event{B_2}{5}}}}  
      {\seq}\assume{{\lthb{\event{S}{2}}{\event{S}{5}}}}  
      {\seq}\assume{{\lthb{\event{S}{3}}{\event{S}{5}}}}  
      ~\seq~\guard{\lthb{1}{5}}})
     }\\
      \!\!~\vee~ \code{\;\,( \atransmit{B_2}{S}{\omsg{v}{Yes}}{s}{6} ~\seq~
      \blueord{\assume{\atransmit{B_2}{S}{}{}{6}}
      {\seq}\assume{{\lthb{\event{B_2}{4}}{\event{B_2}{6}}}}  
      {\seq}\assume{{\lthb{\event{S}{2}}{\event{S}{6}}}}  
      {\seq}\assume{{\lthb{\event{S}{3}}{\event{S}{6}}}}  
        ~\seq~\guard{\lthb{1}{6}}~\seq~}
      }\\
      \code{\!\qquad
      \atransmit{B_2}{S}{\omsg{v}{Addr}}{s}{7} ~\seq~ 
      \blueord{\assume{\atransmit{B_2}{S}{}{}{7}}
      {\seq}\assume{{\lthb{\event{B_2}{6}}{\event{B_2}{7}}}}  
      {\seq}\assume{{\lthb{\event{S}{6}}{\event{S}{7}}}}  
      } ~\seq~
      \blueord{\guard{\lthb{6}{7}}}
      )
      )
      % (B2->S:s(No) \/ B2->S:s(Yes);B2->S:s(Addr))
      }
    \end{array}
  \]
}

The refined specification 
contains information
on observable local events and global
communications, which 
can be used to handle proof obligations on
race-free channels, e.g. \code{\guard{\lthb{3}{4}}}.
When race-freedom cannot be guaranteed, we could also 
introduce explicit synchronization to ensure it. 
%% Moreover, the presence of guards
%% explicitly gives proof obligations that are required
%% to ensure race-freedom over shared channels
%% and message safety over non-deterministic communication.
Unique labels on each transmission, and thus its events,
are trivially
added by our refinement process.

We also generate immediate \code{\precx{HB}} orderings
between each pair of adjacent events of the same party
in the global protocol, as follows:
{\footnotesize
\[
\code{..\assumeL{\event{P}{\atid_1}}{P}.. ~\seq~
  ..\assumeL{\event{P}{\atid_2}}{P}..} \implies
\code{\assume{\lthb{\event{P}{\atid_1}}{\event{P}{\atid_2}}}} 
\]

%% , and safety of
%% non-deterministic communication, e.g \code{\guard{2 \useq 3}}.


%% After some more thought, I think we need to introduce
%% the notion of locally observable events, namely:
%%    +(R1^l)_R1 
%% which denotes that R1^l can be observed by only
%% R1 at its occurrence in the global protocol.

}
  %% ..+(R^l1)_R.. ; ..+(R^l2)_R..
  %%    --> +(R^l1 <_HB R^l2)_R
While the \code{\precx{HB}} and \code{\precx{CB}}
are globally observable events, 
some of them are partial (or dynamic) in nature 
due to the presence of disjunction. Our present
solution to disjunctive formulae is to enforce
a restricted form of disjunction where only 
a common sender and a common receiver
are involved in each disjunctive formula. 
This well-formed restriction ensures that
parties involved in disjunction know precisely which
conditional branches are being executed.
With this restriction,
%% For simplicity,
%% let us first assume the absence of disjunctive 
%% (non-mandated) transmissions. In their absence,
we can soundly use the following 
global propagation lemma since it will always
be transitively undertaken for all branches of
the disjunct.

{\footnotesize
\[\vspace*{-2mm}
\begin{array}{lll}
%% \code{\assume{\lthb{\event{R_1}{\atid_1}}{\event{R_2}{\atid_2}}}}
%% \wedge
%% \code{\assume{\lthb{\event{R_2}{\atid_2}}{\event{R_3}{\atid_3}}}}
%% & \implies & \code{\assume{\lthb{\event{R_1}{\atid_1}}{\event{R_3}{\atid_3}}}} \\
\code{\assume{\lthb{\event{P_1}{\atid_1}}{\event{P_2}{\atid_2}}}}
\wedge
\code{\assume{\lthb{\event{P_2}{\atid_2}}{\event{P_3}{\atid_3}}}}
& \implies & \code{\assume{\lthb{\event{P_1}{\atid_1}}{\event{P_3}{\atid_3}}}} 
\end{array}
\]
}

Another kind of propagation lemmas involve
the \code{\precx{CB}}-ordering.
There are two possible lemmas:
{\footnotesize
\[\vspace*{-2mm}
\begin{array}{lllr}
\code{\assume{\lthb{\event{P_1}{\atid_1}}{\event{S_2}{\atid_2}}}}
\wedge
\code{\assume{\ltcb{\event{S_2}{\atid_2}}{\event{R_3}{\atid_2}}}}
& \implies & \code{\assume{\lthb{\event{P_1}{\atid_1}}{\event{R_3}{\atid_2}}}} & (1)\\
\code{\assume{\ltcb{\event{S_1}{\atid_1}}{\event{R_2}{\atid_1}}}}
\wedge
\code{\assume{\lthb{\event{R_2}{\atid_1}}{\event{P_3}{\atid_2}}}}
& \implies & \code{\assume{\lthb{\event{S_1}{\atid_1}}{\event{P_3}{\atid_2}}}} & (2)
\end{array}
\]
}

Both of these global propagation lemmas, which use the
\code{\precx{CB}} ordering, are sound if 
we assume race-free communication. Under such race-free
condition, the \code{\precx{CB}} ordering behaves in a manner
identical to \code{\precx{HB}}. However,
we are also using these propagation rules
to verify race-freedom by checking if 
proof obligations of the form \code{\guard{\lthb{i_1}{i_2}}} hold.
%% In this proving process, we may use such global propagation
%% lemmas.
As it turns out, only the latter lemma \code{(2)}
is sound for use in ensuring race-freedom, but not
%% the former
 \code{(1)}.
This observation is a novel contribution
of our approach. Let us first explain why
\code{(1)} is unsound to use. Consider two
transmissions over the same channel
\code{(\atransmit{A}{B}{t_1}{\chanvar}{\atid_1})\,\seq\,(\atransmit{C}{D}{t_2}{\chanvar}{\atid_2})}
%% \code{A-1->B ; C-2->D}
. From these transmissions,
we would have
\code{\ltcb{\event{A}{\atid_1}}{\event{B}{\atid_1}}} and
\code{\ltcb{\event{C}{\atid_2}}{\event{D}{\atid_2}}}. 
Consider a scenario where we have already
established \code{\lthb{\event{B}{\atid_1}}{\event{C}{\atid_2}}}.
If \code{(1)} holds,
we could then
conclude \code{\lthb{\event{B}{\atid_1}}{\event{D}{\atid_2}}}. 
However, \code{D} is a party that is independent of \code{B} and \code{C}.
It could thus race ahead of event \code{\event{B}{\atid_1}}.
Hence, \code{(1)} is unsound to use. If \code{(2)} holds,
we can establish \code{\lthb{\event{A}{\atid_1}}{\event{C}{\atid_2}}}.
This holds since its converse \code{\lthb{\event{C}{\atid_2}}{\event{A}{\atid_1}}}
leads to \code{\lthb{\event{C}{\atid_2}}{\event{B}{\atid_1}}}
which contradicted with
our initial assumption. Hence \code{(2)} holds.
With these sound propagation lemmas, we can
generate more %% global
\code{\precx{HB}} orderings
to support better implicit synchronization.


 %% +(R1^l1 <_HB R2^l2) /\ +(R2^l2 <_HB R3^l3)
 %%    --> +(R1^l1 <_HB R3^l3)
 %% +(R1^l1 <_HB R2^l2) /\ +(R2^l2 <_CB R3^l3)
 %%     --> +(R1^l1 <_HB R3^l3)
\hide{
The first lemma captures the transitivity of \code{\precx{HB}}.
The second lemma is novel (or unusual) as it
shows that \code{\precx{CB}} ordering can 
be used only at the start of \code{\precx{HB}} ordering.
This use is sound since we are only stating
\code{\lthb{\event{R_1}{\atid_1}}{\event{R_3}{\atid_3}}} 
but not 
\code{\lthb{\event{R_1}{\atid_1}}{\event{R_2}{\atid_3}}}.
This is the former holds due to our assumption
on \code{\precx{CB}} occurring first. However, the 
latter cannot be guaranteed since we may have 
racy channels.
%% at the beginning we expect
%% the \code{\precx{CB}} to strictly enforce the sender and receiver.
Moreover, it is not possible to have two adjacent
\code{\precx{CB}} orderings, like 
\code{\ltcb{\event{R_1}{\atid_1}}{\event{R_2}{\atid_2}} {\wedge}
\ltcb{\event{R_2}{\atid_2}}{\event{R_3}{\atid_3}}
} since the events of every \code{\precx{CB}} ordering 
are uniquely labelled. Hence, two consecutive 
\code{\precx{CB}} orderings must be separated 
by a \code{\precx{HB}} ordering, as follows:

\code{\ltcb{\event{R_1}{\atid_1}}{\event{R_2}{\atid_2}} 
{\wedge} \lthb{\event{R_2}{\atid_2}}{\event{R_3}{\atid_3}}
{\wedge}
\ltcb{\event{R_3}{\atid_3}}{\event{R_4}{\atid_4}}
{\wedge}
\lthb{\event{R_4}{\atid_3}}{\event{R_5}{\atid_4}}
}

The \code{\precx{HB}} guarantees that \code{\event{R_3}{\atid_3}} 
will occur after \code{\event{R_2}{\atid_2}}, and 
that \code{\event{R_4}{\atid_4}} 
will occur after \code{\event{R_5}{\atid_5}}.

similarly
for The first
\code{\precx{HB}} would ensure \code{\event{R_1}{\atid_1}}
always occur before \code{\event{R_2}{\atid_2}}.
However, we cannot enforce 
\code{\lthb{\event{R_2}{\atid_2}}{\event{R_3}{\atid_3}}} nor
 that \code{ }
}
%% \begin{verbatim}
%% Consider:
%%  A <_CB B ; B <_HB B2  ; X <_CB Y
%% We assume A <_HB B2.
%% However, let us assume a race scenario
%% that looks like below.
%%  A <_CB Y ; B <_HB B2 ; X <_CB B 
%% In this case X <_HB B2, but we cannot really
%% conclude A <_HB B2. Is this an unsoundness
%% of our CB lemma? How can we tighten further?
%%  X <_CB B ;  B <_HB B2 ; A <_CB Y ; 
%% =================================
%% Consider:
%%  A <_CB B ; B <_HB B2  ; X <_CB Y
%% Our propagation lemma
%% allow us to conclude A <_HB B2
%% Assume in a particular scenario to ensure
%% race-freedom, we manages to use B2 <_HB X.
%% to allow us to prove:
%%   A <_HB B2 & B2 <_HB X ==> A <_HB X
%% Can this be confirmed by all execution
%% Another case would be:
%%   A <_HB X
%% We were supposed to prove:
%%  A <_CB B /\ B <_HB B2  X <_CB Y
%% This would have relied on either explicit
%% sync or A<:B2.
%%   A <_HB X & B <_HB Y
%% However, after this proof, we do have
%% A <_HB B2. If we had relied on
%% A <_HB B2, we would again have A<_CB B.
%% =======================================
%%  A1 <_CB A2  /\  B <_HB B2  /\ B2 <_CB Y
%% Can we conclude B <: Y. How can this be used?
%% Assume we have A2<:B. Using it, we can compute
%% A2 <: Y. But is this true? It may not be
%% because Y may have occurred earlier than A2;
%% so that A1 sends to Y instead. Thus, it is not
%% the case that B <_HB Y.
%% ==========================================
%% Consider:
%%  A <_CB B /\ B <_HB C  /\ C <_CB D
%% We can conclude A <_HB C since 
%%  (i) C could only happen after B, and
%%  (ii) A <_CB B requires B to be blocked
%%       till A has completed
%% However, we cannot conclude B <_HB D
%% since both B and D are independent events
%% that can occur in a diff order.
%% Ditto for A and D.
%% Howeveris blocked from /\ C <_CB D /\ D <_HB E
%% From here, we only conclude
%%   A <_HB C  and C <_HB E and A <_HB E and B A <_HB E
%% However, we never conclude:
%%   B <_HB D, nor A <_HB D 
%% The reason for this is that B and D asince race may cause  to happen
%% Race may lead to:
%%  A <_CB D /\ B <_HB C /\ C <_CB B /\ D <_HB E
%%  C <_CB B /\ B <_HB C /\ A <_CB D /\ D <_HB E
%% \end{verbatim}
\wnnay{I think the last lemma is really novel, but I am not sure how to explain properly the
role of \code{\precx{CB}}. \code{A->B;B->C} example
shows that \precx{CB} can only appear at the start}
\wnnay{can we really use \code{\precx{HB}},
and \code{\precx{CB}} and another \code{\precx{CB}}}
\wnnay{We managed to prove that one lemma is sound and the other unsound
in the context of using it to prove race-freedom}

\subsection{Specification Projection}
\wnnay{projection \& automated verification?
Does projection require some global assume/spec that become
available gradually or immediately. For the latter,
is it sound to do so?}

Once we have a specification that has been annotated with assumptions
and obligations, we can proceed to project them for use in
code verification. The projection can be done in two phases. Firstly, on
a per-party basis, and secondly on
a per-channel basis. A per-channel within each party
specification allows us to observe all communication
and proof obligation %% (and assumption)
activities within each channel. We propose to
undertake per-channel
projections on specifications for two
reasons. Firstly, it supports backward compatibility, as an earlier
two-party session logic verification system,
\cite{Florin:IECCS15}, was designed based on per-channel
specifications. Secondly, it is likely
to be easier to add channel-specific quantitative proof
obligation(s), such as boundedness of channel's
buffer \cite{Denielou:2010}, using this approach. However, this topic
is reserved for future investigation.
Furthermore, we also separately project assumptions on
global orderings, that are to be shared by all parties,
%% in a shared space 
so that they may be separately
utilized by each party for their respective
local verification.

Let us first discuss the specification that would
be projected for each party. For the running example,
we would project the following local
specifications for the three parties.

{\footnotesize
  \centering
  \vspace*{-2mm}
  \arraycolsep=1pt
  \[
    \begin{array}{ll}
      \code{\prot{\prj}B_1{\defeq}} & 
      \code{\sendc{s}{}{Order} \seq
      \blueord{\assume{\event{B_1}{1}}} \seq
      \recvc{b_1}{}{Price} \seq
      \blueord{\assume{\event{B_1}{2}}} \seq
      \sendc{b_2}{}{Amt} \seq                          
      \blueord{\assume{\event{B_1}{4}}} \seq
      \blueord{\guard{\lthb{3}{4}}_{B_1}} } \\
      \code{\prot{\prj}B_2{\defeq}} & 
      \code{\recvc{b_2}{}{Price} \seq
      \blueord{\assume{\event{B_2}{3}}} \seq
      \recvc{b_2}{}{Amt} \seq
      \blueord{\assume{\event{B_2}{4}}} \seq
      \blueord{\guard{\lthb{3}{4}}_{B_2}}  \seq}\\
      &\code{
       ((
        \sendc{s}{}{No} \seq                                             
        \blueord{\assume{\event{B_2}{5}}} \seq
        \blueord{\guard{\lthb{1}{5}}_{B_2}}
        ) \vee}\\
      &\code{
        \;\,(\sendc{s}{}{Yes} \seq                                             
         \blueord{\assume{\event{B_2}{6}}} \seq
         \blueord{\guard{\lthb{1}{6}}_{B_2}} \seq
         \sendc{s}{}{Addr} \seq                                             
         \blueord{\assume{\event{B_2}{7}}} \seq
         \blueord{\guard{\lthb{6}{7}}_{B_2}}
        )
       )
     } 
      \\
      \code{\prot{\prj}S{\defeq}} & 
      \code{\recvc{s}{}{Order} \seq
      \blueord{\assume{\event{S}{1}}} \seq
      (\sendc{b_1}{}{Price} \seq
      \blueord{\assume{\event{S}{2}}})
      \useq
      (\sendc{b_2}{}{Price} \seq
      \blueord{\assume{\event{S}{3}}}) \seq
      \blueord{\guard{\lthb{3}{4}}_S}  \seq }\\
      &\code{
       ((
        \recvc{s}{}{No} \seq                                             
        \blueord{\assume{\event{S}{5}}} \seq
        \blueord{\guard{\lthb{1}{5}}_S}
        ) \vee}\\
      &\code{
        \;\,(\recvc{s}{}{Yes} \seq                                             
         \blueord{\assume{\event{S}{6}}} \seq
         \blueord{\guard{\lthb{1}{6}}_S} \seq
         \recvc{s}{}{Addr} \seq                                             
         \blueord{\assume{\event{S}{7}}} \seq
         \blueord{\guard{\lthb{6}{7}}_S}
        )
       )
     }   
     %% \code{~\seq \blueord{\guard{2 \useq 3}}}
      
    \end{array}
  \]
}
\hide{
\begin{verbatim}
B1:
 B1!s;+(B1^1);B1?(b1);+(B1^2);
 B1!b2;+(B1^4);-(3 <_HB 4)_{B1};

B2:
 B2?b2;+(B2^3);
 B2?b2;+(B2^4);-(3 <_HB 4)_{B2};
(B2!s;+(B2^5);-(1 <_HB 5)_{B2};
 \/B2!s;+(B2^6);-(1 <_HB 6)_{B2};B2!s;+(B2^7)-(6 <_HB 7)_{B2})

S:
 S?s;+(S^1);
 (S?b1;+(S^2)*S?b2;+(S^3));-(3 <_HB 4)_S;
(S?s;+(S^5);-(1 <_HB 5)_{S};
 \/S?s;+(S^6);-(1 <_HB 6)_{S};S?s;+(S^7);-(6 <_HB 7)_{S};)
\end{verbatim}
}
Each of the local specification contains send/receive
proof obligations, such as \code{\sendc{s}{}{Order}} and
\code{\recvc{s}{}{Order}},
which capture expected 
channel and message type (or property). It also
contains assumptions on the local events, such as  \code{\assume{\event{B_1}{1}}}
and \code{\assume{\event{S}{1}}} that are immediately released once
the corresponding send/receive obligations have been locally
verified. We may also have global
proof obligations, such as \code{\guard{\lthb{3}{4}}}, 
that is meant to ensure
that the two transmissions, labelled as \code{3} and \code{4},
are race-free since they share a common channel.
This particular global obligation needs to 
be collectively proven after the sender and receiver of transmission \code{4}, namely
\code{B_1} and \code{B_2}, but could be assumed by other parties.
Thus, we project the
relevant portion that has to be proven and assumed 
by the three parties, \code{S, B_1} and \code{B_2}, as
\code{\guard{\lthb{3}{4}}_{B_1}},
\code{\guard{\lthb{3}{4}}_{B_2}} and
\code{\guard{\lthb{3}{4}}_{S}}.
As
\code{\guard{\lthb{3}{4}}}
involves
\code{\guard{(\lthb{\event{S}{3}}{\event{B_1}{4}} 
   %% \vee \lthb{\event{B_2}{3}}{\event{B_1}{4}}
   )
    {\wedge}
    (\lthb{\event{B_2}{3}}{\event{B_2}{4}})}},
these three projections are translated, as follows:
%% \wnsay{should prove before assume}


{\footnotesize
  \centering
  \vspace*{-2mm}
  \arraycolsep=1pt
  \[\vspace*{-2mm}
    \begin{array}{lll}
      \code{\guard{\lthb{3}{4} }_{B_1}} & {=} &
      \code{\guard{\lthb{\event{S}{3}}{\event{B_1}{4}} 
     %% \vee\lthb{\event{B_2}{3}}{\event{B_1}{4}}
     } \seq
      \assume{\lthb{\event{B_2}{3}}{\event{B_2}{4}}} }
      \\
      \code{\guard{\lthb{3}{4} }_{B_2}} & {=} &
      \code{
      \assume{\lthb{\event{S}{3}}{\event{B_1}{4}}} 
      \seq
      \guard{\lthb{\event{B_2}{3}}{\event{B_2}{4}}
      %% \vee\lthb{\event{B_2}{3}}{\event{B_1}{4}}
      } 
      }
      \\
      \code{\guard{\lthb{3}{4} }_{S}} & {=} &
      \code{\assume{\lthb{\event{S}{3}}{\event{B_1}{4}} 
      %% \vee\lthb{\event{B_2}{3}}{\event{B_1}{4}}
      } \seq
      \assume{\lthb{\event{B_2}{3}}{\event{B_2}{4}}} }     
    \end{array}
  \]
}

\hide{
\begin{verbatim}
-(3 <_HB 4)_B1 = -((S^{3} <_{HB} B1^{4} \vee B2^{3} <_{HB} B1^{4}))
    ;+(B2^{3} <_{HB} B2^{4})
-(3 <_HB 4)_B2 =  +(B2^{3} <_{HB} B2^{4})
    ;-((S^{3} <_{HB} B1^{4} \vee B2^{3} <_{HB} B1^{4}));
-(3 <_HB 4)_S =  +(B2^{3} <_{HB} B2^{4})
    ;+((S^{3} <_{HB} B1^{4} \vee B2^{3} <_{HB} B1^{4}));
\end{verbatim}
}

Each party must prove the obligation that is attributable to it, but may
assume the obligations of the other parties.  In the case of
\code{S}, no proof obligation is attributable to it; allowing 
\code{S} to benefit from this
global proof obligation (done by others) as an assumption.
This is %% perhaps
the power of cooperative global proving,
where relevant proof obligations are undertaken locally, but
may otherwise be assumed to hold globally.
%% This particular
%% obligation meant to ensure
%% that the two transmissions, labelled as \code{3} and \code{4},
%% are race-free since they share a common channel.
%% As such global proof obligation have to be proven
%% collectively at two places, after the send and receive of the second 
%% transmission, we use a \code{1/2} fractional permission to denote it.
Such cooperative proving allows us to prove a global obligation,
such as \code{\guard{\lthb{3}{4}}}, at multiple places. 
%% Specifically, we check for
%% ? at ?, and ? at ?. 
%% Each party is expected to handle
%% proof obligation(s) that can be attributed to it, but is allowed
%% to assume the other obligations as assumptions,
%% since these other obligation(s) is
%% concurrently proven by another party.
%% At the joins of the different parties,
%% we could combine the partially proven global proof
%% obligations to give a global guard that have been totally
%% proven, and must therefore hold definitely.

The other global orderings from each transmission,
such as {\cb} 
ordering
like \code{\assume{\ltcb{\event{B_1}{1}}{\event{S}{1}}}}, and 
{\em happens-before} ordering between adjacent events within the same
party, like \code{\assume{\lthb{\event{S}{1}}{\event{S}{2}}}}, are placed in a shared space that
is visible to all parties. As these global ordering
information are modelled for unique events and are also
immutable, we propose to release all orderings in
a single step at the beginning of the protocol for simplicity.
Our proposal to release all global ordering together
as a single assumption is done for simplicity.
Though future orderings are not required to prove 
current global obligations, they never cause any
inconsistency to the current state,
%% do not cause 
%% any prcontradiction to the current program state
but merely
add some new orderings that are available in advance.
\scnay{Should we hide the next sentence?}
\hide{The presence of disjuncts cause imprecision 
which could be rectified by tree-share mechanism
%% Our decision is taken for simplicity, and would also
%% work with the concept of precise disjunction 
that we will
describe in Sec~\ref{}.}

%% each adjacent each such as ? and ? are simply captured
%% The assumptions in this global orderings
%% are guarded ?, so as to  release all constraints that
%% may hold globally in the current time. 
%% This includes ordering 
%% constraints that could be happening concurrently.
%% For example, consider the guard \code{-(not(B1^1 {\wedge} S^1)))}.
%% This guard holds if the current time of the party is
%% neither before the event \code{B1^1} nor the event \code{S^1}.
%%  For the first buyer,
%% \code{B1}, the guard will only hold if the current time 
%% passes the event \code{B1^1}, after the \code{Order} had been sent out.
%% For the second seller
%% \code{S}, the guard will only hold if the current time 
%% has passed the event \code{S^1}.
%% For the second buyer \code{B2}, this guard trivially holds since
%% both events may occur concurrently with it.
%% These guards allow the global constraints to be released 
%% as quickly as possible to each party, but not if the constraint
%% is definitely from a future event.

%% constra global constraints are guarded
%% as
%% Projection to local spec per party
\wnnay{Can we label below as \code{G@All} below?}
\wnnay{should we use ``='' rather than ``:''}

{\footnotesize
  \centering
  \vspace*{-2mm}
  \arraycolsep=1pt
  \[\vspace*{-2mm}
    \code{{\prot}{\prj}{\All}}{\defeq}~\begin{array}[t]{l}
      \code{\assume{\ltcb{\event{B_1}{1}}{\event{S}{1}}} \seq}\\
      \code{((\assume{\lthb{\event{B_1}{1}}{\event{B_1}{2}}} \seq
      \assume{\lthb{\event{S}{1}}{\event{S}{2}}} \seq
      \assume{\ltcb{\event{S}{2}}{\event{B_1}{2}}}) \useq 
      }\\
      \code{\;\,
      (\assume{\lthb{\event{S}{1}}{\event{S}{3}}} \seq
      \assume{\ltcb{\event{S}{3}}{\event{B_2}{3}}})) \seq } \\
      \code{\assume{\lthb{\event{B_1}{2}}{\event{B_1}{4}}} \seq
      \assume{\lthb{\event{B_2}{3}}{\event{B_2}{4}}} \seq
      \assume{\ltcb{\event{B_1}{4}}{\event{B_2}{4}}} \seq} \\
      \code{((
      %% ( \guard{\event{B_2}{5}} \vee \guard{\event{S}{5}}) \seq
      \assume{\lthb{\event{B_2}{4}}{\event{B_2}{5}}} \seq
      \assume{\ltcb{\event{S}{2}}{\event{S}{5}}} \seq
      \assume{\ltcb{\event{S}{3}}{\event{S}{5}}} \seq
      \assume{\ltcb{\event{B_2}{5}}{\event{S}{5}}}
      )}\\
      \code{\vee ~(
      %% ( \guard{\event{B_2}{6}} \vee \guard{\event{S}{6}}) \seq
      \assume{\lthb{\event{B_2}{4}}{\event{B_2}{6}}} \seq
      \assume{\lthb{\event{S}{2}}{\event{S}{6}}} \seq
      \assume{\lthb{\event{S}{3}}{\event{S}{6}}} \seq
      \assume{\ltcb{\event{B_2}{6}}{\event{S}{6}}} \seq} \\
      \code{\;\,\;\, 
      \assume{\lthb{\event{B_2}{6}}{\event{B_2}{7}}} \seq
      \assume{\lthb{\event{S}{6}}{\event{S}{7}}} \seq
      \assume{\ltcb{\event{B_2}{7}}{\event{S}{7}}}
      ))
      }
    \end{array}
  \]
}

\hide{
\begin{verbatim}
Global Constraints:
 +(B1^1 <_CB S^1);
 (+(B1^1 <_CB B1^2);+(S^1 <_HB S^2); +(S^2 <_CB B1^2) 
  * +(S^1 <_HB S^3); +(S^3 <_CB B2^3));
 +(B1^2 <_HB B1^4);+(B2^3 <_HB B2^4); +(B1^4 <_CB B2^4);
((-(B2^5)\/-(S^5));+(B2^4 <_HB B2^5);+(B2^5 <_CB S^5) S?s;+(S^5);
 \/(-(B2^6)\/-(S^6));+(B2^4 <_HB B2^6);+(S^2 <_HB S^6);
   +(S^3 <_HB S^6);+(B2^6 <_CB S^6);
   +(B2^6 <_HB B2^7);+(S^6 <_HB S^7);+(B2^7 <_CB S^7))
\end{verbatim}
}

%% \wnsay{Is the use of guard for disjunction correct?
%% }

%% To summarise our projection process,
Given global specification \code{G} over 
\code{n} parties, \code{P_1{\cdots}P_n},
our projection would %% initially 
transform \code{G} 
into a per-party specification, as follows:
\begin{small}
\[\vspace*{-2mm}
\begin{array}{lcl}
\code{\prot} & \implies & \code{\prot{\prj}P_1} ~{\sep}~ {\cdots} ~{\sep}~\code{\prot{\prj}P_n} ~{\sep}~\code{\prot{\prj}{\All}}
%% \\
%% \code{\prot{\prj}P} & \implies & \code{\perchanprj{\prot}{P}{k_1}} ~{\sep}~ {\cdots} ~{\sep}~\code{\perchanprj{\prot}{P}{k_n}}  
\end{array}
\]
\end{small}
\noindent
where \code{\prot{\prj}P_1~{\sep}~ {\cdots} ~{\sep}~\prot{\prj}P_n} denote the per-party specifications
and \code{\prot{\prj}{\All}} denotes the 
global orderings that are shared by all parties.

Once we have a per-party specification, say \code{\prot{\prj}P_i}
over channels \code{\chanvar_1{\cdots}\chanvar_m}, we can further project
each of these specifications into a
spatial conjunction of several per-channel specifications,
namely \sm{\code{\perchanprj{\prot}{P}{\chanvar_1}{\sep}{\cdots}~{\sep}~\perchanprj{\prot}{P}{\chanvar_m}}}, as follows:
\hide{%
\begin{verbatim}
G    ==> G@P1 * .. * G@Pn * G@All
G@P  ==> G@P<k1> * .. * G@P<kn> 
\end{verbatim}
}%
\begin{small}
\[\vspace*{-2mm}
\begin{array}{lcl}
%% \code{\prot} & \implies & \code{\prot{\prj}P_1} ~{\sep}~ {\cdots} ~{\sep}~\code{\prot{\prj}P_n} ~{\sep}~\code{\prot{\prj}{\All}}
%% \\
\code{\prot{\prj}P_i} & \implies & \code{\perchanprj{\prot}{P_i}{\chanvar_1}} ~{\sep}~ {\cdots} ~{\sep}~\code{\perchanprj{\prot}{P_i}{\chanvar_m}}  
\end{array}
\]\vspace*{-2mm}
\end{small}


For our running example, the seller and two buyers
protocol %% specifications
can be projected into the three channels, as 
follows:

{\footnotesize
  \centering
 % \vspace*{-2mm}
  \arraycolsep=1pt
  \[ \vspace*{-2mm}
    \begin{array}{ll}
      \code{\prot{\prj}B_1{\defeq}} & 
      \code{\sendc{s}{}{Order} \seq
      \blueord{\assume{\event{B_1}{1}}} \seq
      \recvc{b_1}{}{Price} \seq
      \blueord{\assume{\event{B_1}{2}}} \seq
      \sendc{b_2}{}{Amt} \seq                          
      \blueord{\assume{\event{B_1}{4}}} \seq
      \blueord{\guard{\lthb{3}{4}}_{B_1}} } \\
      & \code{\Downarrow (\text{per channel projection})}\\
      & \begin{array}{lll}
          \code{\perchanprj{\prot}{B_1}{s}} & \code{\defeq}&\code{\send{}{Order} \seq
                     \blueord{\assume{\event{B_1}{1}}}}\\
          \code{\perchanprj{\prot}{B_1}{b_1}} & \code{\defeq}& \code{\blueord{\guard{\event{B_1}{1}}} \seq
                       \recv{}{Price} \seq
                       \blueord{\assume{\event{B_1}{2}}}}\\
          \code{\perchanprj{\prot}{B_1}{b_2}} & \code{\defeq} & \code{\blueord{\guard{\event{B_1}{2}}} \seq
                       \send{}{Amt} \seq                          
                       \blueord{\assume{\event{B_1}{4}}} \seq
                       \blueord{\guard{\lthb{3}{4}}_{B_1}} 
                       } 
      \end{array} \\            
      \code{\prot{\prj}B_2{\defeq}} & 
      \code{\recvc{b_2}{}{Price} \seq
      \blueord{\assume{\event{B_2}{3}}} \seq
      \recvc{b_2}{}{Amt} \seq
      \blueord{\assume{\event{B_2}{4}}} \seq
      \blueord{\guard{\lthb{3}{4}}_{B_2}}  \seq}\\
      &\code{
       ((
        \sendc{s}{}{No} \seq                                             
        \blueord{\assume{\event{B_2}{5}}} \seq
        \blueord{\guard{\lthb{1}{5}}_{B_2}}
        ) \vee
        (\sendc{s}{}{Yes} \seq                                             
         \blueord{\assume{\event{B_2}{6}}} \seq
         \blueord{\guard{\lthb{1}{6}}_{B_2}} \seq
         \sendc{s}{}{Addr} \seq                                             
         \blueord{\assume{\event{B_2}{7}}} \seq
         \blueord{\guard{\lthb{6}{7}}_{B_2}}
        )
       )
     } 
      \\
      & \code{\Downarrow (\text{per channel projection})}\\
      & \begin{array}{lll}
          \perchanprj{\prot}{B_2}{b_2} & \code{\defeq} & \code{
                       \recv{}{Price} \seq
                       \blueord{\assume{\event{B_2}{3}}} \seq
                       \recv{}{Amt} \seq
                       \blueord{\assume{\event{B_2}{4}}} \seq
                       \blueord{\guard{\lthb{3}{4}}_{B_2}}
                                  }\\
          \perchanprj{\prot}{B_2}{s} & \code{\defeq} & \code{
                                  \blueord{\guard{\event{B_2}{4}}} \seq
                                  ((
                                  \send{}{No} \seq                                             
                                  \blueord{\assume{\event{B_2}{5}}} \seq
                                  \blueord{\guard{\lthb{1}{5}}_{B_2}}
                                  ) \vee
                       (\send{}{Yes} \seq                                             
                       \blueord{\assume{\event{B_2}{6}}} \seq
                       \blueord{\guard{\lthb{1}{6}}_{B_2}} \seq
                       \send{}{Addr} \seq                                             
                       \blueord{\assume{\event{B_2}{7}}} \seq
                       \blueord{\guard{\lthb{6}{7}}_{B_2}}
                       )
                       )    
                                  }\\
          
      \end{array} \\          
      \code{\prot{\prj}S{\defeq}} & 
      \code{\recvc{s}{}{Order} \seq
      \blueord{\assume{\event{S}{1}}} \seq
      (\sendc{b_1}{}{Price} \seq
      \blueord{\assume{\event{S}{2}}})
      \useq
      (\sendc{b_2}{}{Price} \seq
      \blueord{\assume{\event{S}{3}}}) \seq
      \blueord{\guard{\lthb{3}{4}}_S}  \seq }\\
      &\code{
       ((
        \recvc{s}{}{No} \seq                                             
        \blueord{\assume{\event{S}{5}}} \seq
        \blueord{\guard{\lthb{1}{5}}_S}
        ) \vee (\recvc{s}{}{Yes} \seq                                             
         \blueord{\assume{\event{S}{6}}} \seq
         \blueord{\guard{\lthb{1}{6}}_S} \seq
         \recvc{s}{}{Addr} \seq                                             
         \blueord{\assume{\event{S}{7}}} \seq
         \blueord{\guard{\lthb{6}{7}}_S}
        )
       )
      }\\
      & \code{\Downarrow (\text{per channel projection})}\\
      & \begin{array}{lll}
          \code{\perchanprj{\prot}{S}{b_1}} & \code{\defeq} & \code{
                                 \blueord{\guard{\event{S}{1}}} \seq
                                  \send{}{Price} \seq
                                  \blueord{\assume{\event{S}{2}}}
                                  }\\
          \code{\perchanprj{\prot}{S}{b_2}} & \code{\defeq} & \code{
                                  \blueord{\guard{\event{S}{1}}} \seq
                                  \send{}{Price} \seq
                                  \blueord{\assume{\event{S}{3}}}
                                  \seq
                                  \blueord{\guard{\event{S}{2}}} \seq
                                  \blueord{\guard{\lthb{3}{4}}_S} 
                                  }\\
          \code{\perchanprj{\prot}{S}{s}} & \code{\defeq} & \code{
                                \recv{}{Order} \seq
                                \blueord{\assume{\event{S}{1}}} \seq
                                (\blueord{\guard{\event{S}{2}}} \useq
                                \blueord{\guard{\event{S}{3}}}) \seq
                                }\\
          &&\code{
             ((
             \recv{}{No} \seq                                             
             \blueord{\assume{\event{S}{5}}} \seq
             \blueord{\guard{\lthb{1}{5}}_S}
             ) \vee (\recv{}{Yes} \seq                                             
            \blueord{\assume{\event{S}{6}}} \seq
            \blueord{\guard{\lthb{1}{6}}_S} \seq
            \recv{}{Addr} \seq                                             
            \blueord{\assume{\event{S}{7}}} \seq
            \blueord{\guard{\lthb{6}{7}}_S}
            )
            )
        }\\
          
        \end{array} \\ 
     %% \code{~\seq \blueord{\guard{2 \useq 3}}}
      
    \end{array}
  \]
}

Each of these per-channel specification
may actually 
contain event guards, such as
\code{\blueord{\guard{\event{S}{1}}}}. These guards on events 
are important for ensuring that
send/receive operations over different
channels but within the same party
are correctly synchronized. 
For example, we require that \code{\recv{s}{Order}}
be executed before \code{\send{b_1}{Price}} 
within party \code{S}, and this is
ensured by placing
\code{\blueord{\guard{\event{S}{1}}}}
before \code{\send{b_1}{Price}}.
\hide{
\begin{verbatim}
B1:
 B1!s;+(B1^1);B1?(b1);+(B1^2);
 B1!b2;+(B1^4);-(3 <_HB 4)_{B1}
=channel=>
 s: B1!s;+(B1^1));
 b1: -(B1^1);B1?(b1);+(B1^2);
 b2: -(B1^2)B1!b2;+(B1^4);-(3 <_HB 4)_{B1};

B2:
 B2?b2;+(B2^3);
 B2?b2;+(B2^4);-(3 <_HB 4)_B2;
(B2!s;+(B2^5);-(1 <_HB 5)_B2;
 \/B2!s;+(B2^6);-(1 <_HB 6)_B2;B2!s;+(B2^7);-(6 <_HB 7)_B2)
=channel=>
 b2: B2?b2;+(B2^3);B2?b2;+(B2^4);-(3 <_HB 4)_B2;
 s:  -(B2^4);
      (B2!s;+(B2^5)-(1 <_HB 5)_B2; 
      \/B2!s;+(B2^6);-(1 <_HB 6)_B2;B2!s
         ;+(B2^7);-(6 <_HB 7)_B2)

S:
 S?s;+(S^1);
 (S?b1;+(S^2)*S?b2;+(S^3));+(3 <_HB 4);
(S?s;+(S^5);-(1 <_HB 5)_{S} 
 \/S?s;+(S^6);-(1 <_HB 6)_{S};S?s;+(S^7);-(6 <_HB 7)_{S})
=channel=>
 b1: -(S^1);(S?b1;+(S^2));
 b2: -(S^1);(S?b2;+(S^3));-(S^2);+(3 <_HB 4);
 s: S?s;+(S^1);-(S^2)*-(S^3);
    (S?s;+(S^5);-(1 <_HB 5)_{S} 
     \/S?s;+(S^6);-(1 <_HB 6)_{S};S?s;+(S^7);-(6 <_HB 7)_{S})
\end{verbatim}
}


\subsection{Automated Local Verification}
Once we have the refined specification that had been 
suitably projected on a per party and per channel
basis, we can proceed to
use these specifications for automated local verification.
The shared global orderings can be immediately added to the 
initial program state.  The per-channel specification 
are released during the verification on each of the respective
program codes, namely \code{(Code_S ~||~ Code_{B_1} ~||~ Code_{B_2})},
for the different parties. For our running example,
the initial and final program states are:

\hide{%
\begin{verbatim}
{ Common(G#All) * Party<S,G#S> * Party<B1,G#B1> 
  * Party<B2,G#B2> }
   (Code_S ~||~ Code_{B1} ~||~ Code_{B2}) 
{ Party<S,emp> * Party<B1,emp> * Party<B2,emp> }
\end{verbatim}
}%
{\footnotesize
\[ \vspace*{-2mm}
\begin{array}{c}
\{\commonspec{{\prot}{\prj}{\All}} ~{\sep}~\partyspec{S}{{\prot}{\prj}{S}} ~{\sep}~\partyspec{B_1}{{\prot}{\prj}{B_1}} 
~{\sep}~\partyspec{B_2}{{\prot}{\prj}{B_2}}\}
\\
\code{(Code_S ~||~ Code_{B_1} ~||~ Code_{B_2})}
\\
\{\partyspec{S}{\emp} ~{\sep}~\partyspec{B_1}{\emp} 
~{\sep}~\partyspec{B_2}{\emp}\}
\end{array}
\]
}


The \code{\emp} in the final state of each
party can help to confirm the completion of
all transmissions in
the global protocol. The abstract predicate \code{\partyspec{S}{{\prot}{\prj}{S}}}
associates each party with its corresponding specification. 
Our approach supports both events that are either
{\em immutable} or {\em mutable}. %% As seen earlier, 
Each immutable event (seen earlier)
is %% always
labelled uniquely, while mutable
events can be updated flow-sensitively.
To signify each executing party \code{P}, we use
a mutable event \code{\peer{\rolevar}} that is
updated when \code{\rolevar} is executing. Such mutable events are
added to %% our code
as ghost specifications, as shown below.
\hide{
We can also guide 
and restrict the use of each party's specification
%% to the respective parties 
by the use on
guards and assumptions on each party, 
such as \code{\guard{B_1}} and \code{\assume{B_1}}
for party \code{B_1},
as shown below.
}
\hide{
\asay{can we only keep one initial state in the below? (with either
  \code{\commonspec{{\prot}{\prj}{\All}}}
  or
   \code{{\prot}{\prj}{\All}} ?
   )}
\asay{
   Why is +(S), +(B1), etc part of the code?}
\asay{
   It looks like the orders disappeared from the poststate.}
\asay{
 I wonder whether we should support an operation which filters the
   non-orders from a spec, not to be used in reasoning, but
   just for illustration purpose, to emphasizing the poststate of S
   for example: \code{({\prot}{\prj}{S}) \% O \wedge {\prot}{\prj}{\All}} }
\asay{
  Should I add +(P).. as part of the language?
}
}
\hide{
\begin{verbatim}
{ Common(G#All) * Party<S,-S;G#S> * Party<B1,-B1;G#B1> 
  * Party<B2,-B2;G#B2> }
{ Party<S,-G;G#S> * Party<B1,-B1;G#B1> * Party<B2,-B2;G#B2> & G$All }
 ( {Party<S,-G;G#S> & G#All} +S;Code_S {Party<S,emp> & ?}
  ~||~ 
   {Party<B_1,-B1;G#B_1> & G#All} 
       +B1;Code_{B1}  {Party<B_1,emp> & ?}
  ~||~ 
   {Party<B_1,-B2;G#B_2> & G#All} 
       +B2;Code_{B2}  {Party<B_2,emp> & ?}
 ) 
{ Party<S,emp> * Party<B1,emp> * Party<B2,emp> & ? }
{ Party<S,emp> * Party<B1,emp> * Party<B2,emp> }
\end{verbatim}
}

{\footnotesize
\[ \vspace*{-2mm}
\begin{array}{c}
\{\commonspec{{\prot}{\prj}{\All}} ~{\sep}~\partyspec{S}{{\prot}{\prj}{S}} ~{\sep}~\partyspec{B_1}{{\prot}{\prj}{B_1}} 
~{\sep}~\partyspec{B_2}{{\prot}{\prj}{B_2}}\}
\\
\{\partyspec{S}{{\prot}{\prj}{S}} ~{\sep}~\partyspec{B_1}{{\prot}{\prj}{B_1}} 
~{\sep}~\partyspec{B_2}{{\prot}{\prj}{B_2}} ~{\wedge}~ \code{{\prot}{\prj}{\All}} 
\}
\\ \\
\left( \begin{array}{l}
\code{ \{\partyspec{S}{{\prot}{\prj}{S}}~{\wedge}~ \code{{\prot}{\prj}{\All}} \} 
\code{~\;\blueord{\assume{\peer{S}}};Code_S~}
\{\partyspec{S}{\emp} ~{\wedge}~ \hov_S\} }
\\
\code{~||~}
\\
\code{ \{\partyspec{B_1}{{\prot}{\prj}{B_1}}~{\wedge}~ \code{{\prot}{\prj}{\All}} \} 
\code{~\blueord{\assume{\peer{B_1}}};Code_{B_1}}
\{\partyspec{B_1}{\emp} ~{\wedge}~ \hov_{B_1}\} }
\\
\code{~||~}
\\
\code{ \{\partyspec{B_2}{{\prot}{\prj}{B_2}}~{\wedge}~ \code{{\prot}{\prj}{\All}} \} 
\code{~\blueord{\assume{\peer{B_2}}};Code_{B_2}}
\{\partyspec{B_2}{\emp} ~{\wedge}~ \hov_{B_2}\} }
\end{array}
\right)
\\ \\
\code{ \{\partyspec{S}{\emp} ~{\sep}~\partyspec{B_1}{\emp} 
~{\sep}~\partyspec{B_2}{\emp}~{\wedge}~ \hov_S {\wedge}  \hov_{B_1}
  {\wedge}  \hov_{B_2} \} }
\\
\{\partyspec{S}{\emp} ~{\sep}~\partyspec{B_1}{\emp} 
~{\sep}~\partyspec{B_2}{\emp}\}
\end{array} 
\]
}\\


Lastly, to support local verification, we allow the per-channel
specification to be released by
lemmas of the form:
\wnnay{should we use \code{G\#B1\#b1} instead of \code{G\#B1<b1>}}
\scnay{the macro perchanprj is changed to reflect this}
\hide{%
\begin{verbatim}
 Party<B_1,G#B_1> <=> Channel<s,B_1,G#B_1<s>> 
    * Channel<b1,B_1,G#B_1<b1>> 
    * Channel<b2,B_1,G#B_1<b2>>
\end{verbatim}
}%
{\footnotesize
\[
\code{\partyspec{B_1}{{\prot}{\prj}{B_1}} ~{\Leftrightarrow}~ \chanspec{s}{B_1}{\perchanprj{\prot}{B_1}{s}} ~{\sep}~
\chanspec{b_1}{B_1}{\perchanprj{\prot}{B_1}{b_1}} ~{\sep}~
\chanspec{b_2}{B_1}{\perchanprj{\prot}{B_1}{b_2}}}
\]\vspace*{-2mm}
}

On completion, we also have a set of 
lemmas over the \code{emp} state to signify completion
of protocol. An example is shown below:
\hide{%
\begin{verbatim}
 Party<B_1,emp> <=> Channel<s,B_1,emp> 
    * Channel<b1,B_1,emp> * Channel<b2,B_1,emp>
\end{verbatim}
}%
\begin{footnotesize}
\[\vspace*{-2mm}
\code{
\partyspec{B_1}{\emp} ~{\Leftrightarrow}~ \chanspec{s}{B_1}{\emp} ~{\sep}~
\chanspec{b_1}{B_1}{\emp} ~{\sep}~
\chanspec{b_2}{B_1}{\emp}}
\]
\end{footnotesize}

With the help of these lemmas, we can now % perform
allow local verification to proceed, as follows:
\hide{%
\begin{verbatim}
   {Party<B_1,G#B_1> & G#All} 
   {Channel<s,B_1,G#B_1<s>> * Channel<b1,B_1,G#B_1<b1>> 
    * Channel<s,B_1,G#B_1<b2>> & G#All} 
       Code_{B_1}  
   {Channel<s,B_1,emp> * Channel<b1,B_1,emp 
    * Channel<s,B_1,emp> & ?} 
   {Party<B_1,emp> & ?} 
   {Party<B_1,emp>}
\end{verbatim}
}%
\begin{footnotesize}
\[ \vspace*{-2mm}
\begin{array}{c}
\{\partyspec{B_1}{{\prot}{\prj}{B_1}} ~{\wedge}~ \code{{\prot}{\prj}{\All}} \}
\\
\code{\{\chanspec{s}{B_1}{\perchanprj{\prot}{B_1}{s}} ~{\sep}~
\chanspec{b_1}{B_1}{\perchanprj{\prot}{B_1}{b_1}} ~{\sep}~
\chanspec{b_2}{B_1}{\perchanprj{\prot}{B_1}{b_2}}
~{\wedge}~ \code{{\prot}{\prj}{\All}} \}}
\\
\code{\blueord{\assume{\peer{B_1}}};\code{Code_{B_1}}}
\\
\code{\{ \chanspec{s}{B_1}{\emp} ~{\sep}~
\chanspec{b_1}{B_1}{\emp} ~{\sep}~
\chanspec{b_2}{B_1}{\emp}
~{\wedge}~ \hov_{B_1} \}}
\\
\code{\{\partyspec{B_1}{\emp} ~{\wedge}~ \hov_{B_1}\}}
\\
\code{\{\partyspec{B_1}{\emp}\}}
\end{array} 
\]
\end{footnotesize}
\scnay{We still have ? in the above}
%% This is intended for the following program with 
%% codes for the three parties running concurrently:
%% \code{ (Code_S ~||~ Code_{B_1} ~||~ Code_{B_2}) } 
\wnnay{Do we need to talk about how assumptions are released}
\wnnay{Do we need to indicate a flow-sensitive event on parties}

\hide{
\begin{verbatim}

{Initial State} S || B1 || B2 {Final State}




Channels are resources, but events
(that have occurred) and orderings (past and future) are pure info
that can be freely duplicated.

Final state would ensure that every channel
has been completed, and thus fully
complied with the global protocol.

Though we can handle also deadlock-freedom, this
aspects is not discussed in the current paper.

Release of resources and guards..

Local verification on send/receive ..

\end{verbatim}
}
%% A-1->C:(k); A-2->B(k2); B-3->C:(k)

%% Refined Spec
%% ------------
%% A-1->C:(k); +(A^1);+(C^1); +(A^1 <_CB C^1);
%% A-2->B:(k2); +(A^2);+(B^2); +(A^1 <_HB A^2); +(A^2 <_CB B^2);
%% B-3->C:(k); +(B^3);+(C^3); +(B^2 <_HB B^3)
%%    ; +(C^1 <_HB C^3); +(B^3 <_CB C^3); -(1 <_HB 3))

%% Per-Party Projection
%% --------------------
%% A = !k; +(A^1); !k1; +(A^2); -(1 <_HB 3)_A
%% B = ?k1; +(B^2); !k; +(B^3); -(1 <_HB 3)_B
%% C = ?k; +(C^1); ?k; +(C^3); -(1 <_HB 3)_C
%% All: +(A^1 <_CB C^1); +(A^1 <_HB A^2); +(A^2 <_CB B^2)
%%      ; +(B^2 <_HB B^3); +(C^1 <_HB C^3); +(B^3 <_CB C^3); 

%% Per-Channel Projection
%% --------------------
%% A = 
%%    k : !k; +(A^1); 
%%    k1 : -(A^1); !k1; +(A^2); //-(1 <_HB 3)_A
%%          +(A^1 <_HB B_3);+(C^1 <_HB C^3)

%% B = 
%%    k1: ?k1; +(B^2); 
%%    k:  -(B^2); !k; +(B^3); //-(1 <_HB 3)_B
%%        -(A^1 <_HB B_3);+(C^1 <_HB C^3)

%% C = 
%%    k: ?k; +(C^1); ?k; +(C^3); // -(1 <_HB 3)_C
%%        -(C^1 <_HB C^3);+(A^1 <_HB B_3)

\input{disjunct}


==> partial-disj.tex <==
\subsection{Precise Partial Ordering with Tree-Share}

The presence of disjunction in global protocol leads
to partial orderings that are true for only
some of the time. Its presence is akin to
{\em maybe-ordering} rather than {\em must-ordering} since
the ordering only holds if relevant part(s) of the
protocol were executed. However, maybe-ordering is
rather imprecise. To support a precise version of
partial ordering, we propose to use a recent fractional
permission mechanism, known as {\em tree-shares} \cite{Hobor:treeshare}
which was used to characterize a
precise form of fractional ownership.
In our case, we use it to precisely characterize the portion
of time when a partial ordering is expected to hold.
With this use of such a precise fractional mechanism,
our partial ordering information can now be used to obtain
precise global ordering on a {\em conditional-must} 
(synchronized across multiple parties) rather than 
just {\em maybe} basis.

Consider the following example protocol,
%\begin{verbatim}
%  T1;(T2\/ emp);T3
%\end{verbatim}
\sm{\code{T_1;~(T_2 {\vee} \emp);~T_3}}, 
%% \noindent
with three transmissions over  shared common channel, say \code{k}.
If we capture the ordering via adjacent transmissions
as two maybe-orderings, we will obtain
\code{\lthbmay{T_1}{T_2}} and \code{\lthbmay{T_2}{T_3}}  whose transitivity
leads to another imprecise maybe-ordering\code{\lthbmay{T_2}{T_3}}. To capture 
more precise partial ordering, we propose to use tree-shares
where full permission is denoted by \code{\atFull}
and half permission is denoted by either \code{{\at}L=\atL} or \code{{\at}R=\atR}
where \code{{\at}L} and \code{{\at}R} are short-hands for the
two distinct (left and right) 
halves of a full tree-share. Quarter permissions would
thus be either \code{{\at}L{\at}L=\atLL}, \code{{\at}L{\at}R=\atLR},
\code{{\at}R{\at}L=\atRL} or \code{{\at}R{\at}R=\atRR}, giving us precisely
which quarter permission it belongs to. Using it,
we can now label the different transmissions %% more precisely
to indicate which disjunctive branches
each transmission belongs to. Our example
can now be annotated to indicate when each
transmission happens. 

\wnsay{Do we need to uniquely label the disjunction?
Can we show how it works for our running example??}

%\begin{verbatim}
%  T1@1;(T2@(1,0)\/ emp);T3@1
%\end{verbatim}

%\[
\sm{\code{T_1{\atFull};~(T_2{\atL} \,{\vee}\, \emp);~T_3{\atFull}}}
%\]

\code{T1\atFull} states that
its transmission always happens, while \code{T2\atL}
indicates it happens when the left part of its
outer disjunct holds.
%% roughly half the time.
Using this,
the partial ordering we extract as
proof obligations are
\code{\guard{\lthb{T_1\atFull}{T_2\atL}}} and
\code{\guard{\lthb{T_2\atL}{T_3\atFull}}}, which 
states precisely when these two partial orderings 
are expected to hold. We also extract another
adjacent proof obligation
\code{\guard{\lthb{T_1\atFull}{T_3\atFull}}}.
However, part of this obligation
\code{\guard{\lthb{T_1\atFull}{T_3\atL}}} 
can be guaranteed from the previous
two proof obligations (which have become assumptions
after their respective proofs)
using
the following propagation rule (overloaded over events and transmissions):
%% directly 
%% since they are not
%% adjacent due to an intermediate \code{T_2\atL}.
%% (This restriction helps minimise
%% on explicit synchronization needed.)
%% Our main propagation rule is now:
%
\[
\begin{array}{l}
%% \code{\assume{\lthb{\eventf{R_1}{\atid_1}{f1}}{\eventf{R_2}{\atid_2}{f2}}}}
%% \wedge
%% \code{\assume{\ltcb{\eventf{R_2}{\atid_2}{f3}}{\eventf{R_3}{\atid_3}{f4}}}} \\
%% ~~\implies \code{\assume{\lthb{\eventf{R_1}{\atid_1}{f1}}{\eventf{R_3}{\atid_3}{(f2{\wedge}f4)}}}} \\
%% \code{\assume{\lthb{\eventf{R_1}{\atid_1}{f_1}}{\eventf{R_2}{\atid_2}{f_2}}}}
%% \wedge
%% \code{\assume{\lthb{\eventf{R_2}{\atid_2}{f_2}}{\eventf{R_3}{\atid_3}{f_3}}}} \\
%% ~~\implies \code{\assume{\lthb{\eventf{R_1}{\atid_1}{f_1}}{\eventf{R_3}{\atid_3}{(f_2{\wedge}f_3)}}}} \\
\code{\assume{\lthb{\transf{T_1}{\atid_1}{f_1}}{\transf{T_2}{\atid_2}{f_2}}}}
\wedge
\code{\assume{\lthb{\transf{T_2}{\atid_2}{f_2}}{\transf{T_3}{\atid_3}{f_3}}}} \\
~~\implies \code{\assume{\lthb{\transf{T_1}{\atid_1}{f_1}}{\transf{T_3}{\atid_3}{(f_2{\wedge}f_3)}}}} \\
\end{array}
\]

With this propagation of partial ordering assumptions (that may come
from prior proof obligations), we 
are now left with the following proof obligation:
\code{\guard{\lthb{T_1\atFull}{T_3\atR}}}.
Our propagation rules for assumptions
are overloaded for both send/receive
events and transmissions over common channels.
\wnnay{if we always add virtual points for 
missing transmissions in disjunct, the use of tree-share 
may become redundant. This may eliminate the need for
tree-share which makes out scheme simpler.
Is there another use of tree-shares? What is
its real purpose? For \sm{\code{T_1;~(T_2 {\vee} \emp);~T_3}},
we would add \sm{\code{T_1;~(T_2 {\vee} vT_{2b});~T_3}} 
where \sm{vT_{2b}} is a virtual transmission. Using this approach
ordering are no longer partial and are always total with respect
to the latest events.
}
%% Using them, we are able to derive
%% the following partial but precise
%% ordering,
%% \code{\lthb{T_1\atFull}{T_3\atL}}. This 
%% partial %% relation is a precise
%% ordering %% which
%% holds when \code{\atL} disjunctive
%% branch is traversed.
Let us consider slightly different configuration
with \code{T  } denoting either distinct
events or distinct transmissions over common channels.
%% lobal
%% protocol, say:
%% that the ordering holds
%% only partially.

%\begin{verbatim}
%  T1@1;(T2a@(1,0)\/ T2b@(0,1));T3@1
%\end{verbatim}

\sm{\code{T_1{\atFull};~(T_{2a}\atL \vee T_{2b}\atR);~T_3\atFull}}

Assume we can either derive (or prove) the following
partial orderings \code{\lthb{T_1\atFull}{T_{2a}\atL}},
 \code{\lthb{T_1\atFull}{T_{2b}\atR}}, \code{\lthb{T_{2a}\atL}{T_{3}\atFull}}
and \code{\lthb{T_{2b}\atR}{T_{3}\atFull}}.
Using the earlier transitive
propagation rules over partial
orderings, 
we should now be able to derive both
\code{\lthb{T_1\atFull}{T_3\atL}} and \code{\lthb{T_1\atFull}{T_3\atR}}.
%% using the intermediate transmissions \code{T_{2a}\atL} 
%% and \code{T_{2b}\atR}, respectively.
These two partial orderings can be combined
into \code{\lthb{T_1\atFull}{T_3\atFull}}
by the 
conjunctive rule:
%
\[
\begin{array}{l}
\code{\assume{\lthb{\eventf{R_1}{\atid_1}{f_1}}{\eventf{R_2}{\atid_2}{f_2}}}}
\wedge
\code{\assume{\lthb{\eventf{R_1}{\atid_1}{f_1}}{\eventf{R_2}{\atid_2}{f_3}}}} \\
~~\iff \code{\assume{\lthb{\eventf{R_1}{\atid_1}{f_1}}{\eventf{R_2}{\atid_2}{(f_2{\vee}f_3)}}}} \\
\end{array}
\]

This must \code{\precx{HB}} ordering holds
at full permission
\code{\atFull} since the
two disjunctive
branches together ensured it. As partial orderings
derived using tree-share permissions are precise,
they can be used to support global synchronization
locally.

\begin{small}
\[
\begin{array}{ll}
(0,0)              = 0  &\qquad
(1,1)              = 1
\\
\code{f_1 ~{\wedge}~ f_2           = f_2 ~{\wedge}~ f_1}  &\qquad
0 ~{\wedge}~ \_             = 0
\\
\code{(f_1,f_2) ~{\wedge}~ (f_3,f_4) = (f_1{\wedge}f_3,f_2{\wedge}f_4)}  &\qquad
\code{1 ~{\wedge}~ x             = x}
\\
\code{f_1 ~{\vee}~ f_2           = f_2 ~{\vee}~ f_1} &\qquad 
1 ~{\vee}~ \_             = 1
\\
\code{(f_1,f_2) ~{\vee}~ (f_3,f_4) = (f_1{\vee}f_3,f_2{\vee}f_4)} &\qquad
\code{0 ~{\vee}~ x             = x}
\end{array}
\]
\end{small}

\hide{%
\begin{verbatim}
(0,0)              = 0
(1,1)              = 1

f1 /\ f2           = f2 /\ f1
0 /\ _             = 0
1 /\ x             = x
(f1,f2) /\ (f3,f4) = (f1/\f3,f2/\f4)

f1 \/ f2           = f2 \/ f1
1 \/ _             = 1
0 \/ x             = x
(f1,f2) \/ (f3,f4) = (f1\/f3,f2\/f4)
\end{verbatim}
}%
\scnay{Do we need to define \code{f_1{\wedge}f_2} and \code{f_1{\vee}f_2} for tree-shares \code{f_1} and \code{f_2}? What does a zero permission (e.g. \code{(1,0){\wedge} (0,1)}) indicate?}


\wnsay{synchronized disjunction}

\hide{
Outline of all the main steps:
\begin{itemize}
\item collect proof obligations safety
\item insert them in the protocol
\item project the global protocol into local protocol while also
  adding fidelity proof obligations
\item annotate each method correspondingly
\item annotate each ES (eg cdl) correspondingly - a bit tricky since it
  needs to capture labels as well...
\item verify the program using lemmas to release orderings in the
  state
\end{itemize}  
\asay{can choose to analyze safety from the global protocol alone if
concurrency is achieved solely with message passing}
}
%% global propertyover a single shared channel.
%% disjunction leads to dynamic information
%% partial-ordering
%% precise ordering through tree-share




==> recursion.tex <==



==> th_notation.tex <==
\definecolor{darkgreen}{HTML}{008000}

\newcommand{\cb}{{{communicates-before}}}
\newcommand{\hb}{{{happens-before}}}
\newcommand\commonspec[1]{\code{Common(#1)}}
\newcommand\partyspec[2]{\code{Party(#1,#2)}}
\newcommand\gloabspec[3]{\code{Glob(#1,#2,#3)}}
% \newcommand\chanspec[3]{\code{Channel{\langle}#1,#2,#3{\rangle}}}
%\newcommand{\perchanprj}[3]{\code{{#1}{\prj}{#2}{\langle}{#3}{\rangle}}}
\newcommand{\perchanprj}[3]{\code{{#1}{\prj}{#2}{\prj}{#3}}}
\newcommand{\perpartyprj}[2]{\code{{#1}{\prj}{#2}}}
\newcommand{\All}{\code{All}}
\newcommand{\prj}{\mytt{\#}}
\newcommand{\chpred}[2]{{\cal C}(#1,#2)}
\newcommand{\wnsay}[1]{{{\color{blue}({\bf WN:} \textit{#1})}}}
\newcommand{\wnnay}[1]{}
\newcommand{\asay}[1]{{{\color{darkgreen}{\bf A:} \textit{#1}}}}
\newcommand{\anay}[1]{}
\newcommand{\scsay}[1]{{{\color{cyan}({\bf SC:} \textit{#1})}}}
\newcommand{\scnay}[1]{}
\newcommand{\doubt}[1]{{\color{red}{#1}}}
\newcommand{\betw}[1]{\ensuremath{{\cdots}#1{\cdots}}}
\def\defeq{\ensuremath{\,\triangleq}}
\def\cd{\,{\cdot}\,}
\def\compl{{\sim}}
\def\pst{\omega}
\def\st{\ensuremath{\sigma}}
\def\sta{\ensuremath{\sigma'}}
\def\stap{\ensuremath{\sigma''}}
\def\St{\ensuremath{\mathrm{\Delta}}}
\def\Sta{\ensuremath{\mathrm{\Delta'}}}

\def\mw{\ensuremath{-\hspace{-1ex}\circledast~}}

\def\Q{\ensuremath{\code{Q}}}
\def\P{\ensuremath{\code{P}}}
\def\Pow{\ensuremath{\mathcal{P}}}
\def\B{\ensuremath{\mathsf{B}}}
\def\S{\ensuremath{\mathcal{S}}}
\def\SH{\ensuremath{\mathsf{SH}}}
\def\PSH{\ensuremath{\Pow_\SH}}

%\newcommand{\rearr}[2]{\ensuremath{\mathsf{rearr}(#1)(#2)}}
\newcommand{\filter}[2]{\ensuremath{\mathsf{filter}(#1)(#2)}}
%\newcommand{\exec}[2]{\ensuremath{\mathsf{exec}(#1)(#2)}}
%\newcommand{\abs}[1]{\ensuremath{\mathsf{abs}(#1)}}

\def\AllSpec{\ensuremath{\mathsf{AllSpec}}}
\def\T{\ensuremath{\mathcal{T}}}
\def\Pt{\ensuremath{\mathcal{P}^\top}}

\def\rearr{\ensuremath{\mathsf{unfold}}}
\def\exec{\ensuremath{\mathsf{exec}}}
\def\abs{\ensuremath{\mathsf{abs}}}
\def\absa{\ensuremath{\mathsf{abs_a}}}

\def\Rearr{\ensuremath{\mathsf{Unfold}}}
\def\Exec{\ensuremath{\mathsf{Exec}}}
\def\Abs{\ensuremath{\mathsf{Abs}}}

\newcommand{\Pre}{\ensuremath{\mathsf{Pre}}}
\newcommand{\Post}{\ensuremath{\mathsf{Post}}}
\newcommand{\Curr}{\ensuremath{\mathsf{Curr}}}

\def\svar{\ensuremath{\mathsf{svars}}}
\def\rec{\ensuremath{\mathsf{rec}}}
\def\Pairs{\ensuremath{\mathsf{Pairs}}}
\def\Spec{\ensuremath{\mathsf{Spec}}}
\def\mspec{\ensuremath{\myit{mspec}}}
\newcommand{\fv}[1]{\ensuremath{\mathsf{fv}(#1)}}
\newcommand{\lv}[1]{\ensuremath{\mathsf{lv}(#1)}}
\def\Refine{\ensuremath{\mathsf{Refine}}}
\def\ReachVar{\ensuremath{\mathsf{ReachVar}}}
\def\b{\ensuremath{\mathsf{b}}}
\newcommand{\old}[1]{\ensuremath{\mathsf{old}(#1)}}
\newcommand{\ol}[1]{\ensuremath{#1^*}}
\newcommand{\lift}[1]{\ensuremath{#1^\dag}}

\newcommand{\mtt}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\mbf}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\msf}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\sevent}[2]{\ensuremath{#1^{#2}_S}}
\newcommand{\revent}[2]{\ensuremath{#1^{#2}_R}}
\newcommand{\event}[2]{\ensuremath{#1^{(#2)}}}
\newcommand{\eventf}[3]{\ensuremath{#1^{#2}{{\at}#3}}}
\newcommand{\transf}[3]{\ensuremath{#1{{\at}#3}}}

%\newcommand{\pre}[1]{\ensuremath{\mathsf{Pre}_\mtt{#1}}}
%\newcommand{\post}[1]{\ensuremath{\mathsf{Post}_\mtt{#1}}}

\def\Var{\ensuremath{\mathsf{Var}}}
\def\LVar{\ensuremath{\mathsf{LVar}}}
\def\SVar{\ensuremath{\mathsf{SVar}}}

\def\nul{\texttt{null}}

\newcommand{\denoleft}{\ensuremath{|\hspace{-.06cm}[}}
\newcommand{\denoright}{\ensuremath{]\hspace{-.06cm}|}}
\newcommand{\semantic}[3]{{\denoleft}#1{\denoright}_{#2}#3}
\newcommand{\semantica}[3]{{\denoleft}#1{\denoright}_{#2}^\msf{A}#3}
\newcommand{\semantici}[3]{{\denoleft}#1{\denoright}_{#2}#3}
\newcommand{\triple}[3]{\{ #1 \}~ {\color{blue}{#2}} ~\{ #3 \}}

\def\vl{\ensuremath{\mathsf{val}}}
\def\rf{\ensuremath{\mathsf{ref}}}
\def\dispose{\ensuremath{\mathsf{dispose}}}
\def\new{\ensuremath{\mathsf{new}}}
\def\cskip{\ensuremath{\mathsf{skip}}}
\newcommand{\cif}[3]{\ensuremath{\mathsf{if}~#1~\mathsf{then}~#2~\mathsf{else}~#3~\mathsf{fi}}}
\newcommand{\cwhile}[2]{\ensuremath{\mathsf{while}~#1~\mathsf{do}~#2~\mathsf{od}}}
\def\known{\ensuremath{\mathsf{known}}}
\def\unknown{\ensuremath{\myit{unk}}}
\def\local{\ensuremath{\mathsf{local}}}
\def\return{\ensuremath{\mathsf{return}}}

\def\D{\Delta}
\def\Pst{\Upsilon}
\def\S{\mathsf{S}}
\def\H{\mathsf{H}}
\def\Re{\mathsf{R}}
\def\subst{\rho}
\newcommand{\hyphen}[0]{\ensuremath{\mbox{-}}}
\newcommand{\pair}[2]{\ensuremath{(#1, #2)}}%{\ensuremath{\langle #1;~ #2 \rangle}}
\newcommand{\unk}[2]{\ensuremath{\myit{unk}_{#1}{(#2)}}}

\def\TODO{\textsf{TODO}~}

%%%%%%

\def\State{\ensuremath{\varsigma}}
\def\mem{\code{heap}}
\def\stk{\code{stk}}
\def\so{\textit{sizeof}}
\def\sso{\textit{ssizeof}}
\newcommand{\hp}{\ensuremath{\mu}}
\newcommand{\sk}{\ensuremath{\sigma}}
\newcommand{\err}{\ensuremath{\myit{er}}}
\newcommand{\memerr}{\ensuremath{\myit{er}_1}}
\newcommand{\othererr}{\ensuremath{\myit{er}_2}}
%\newcommand{\incsk}[1]{\ensuremath{\stk{:=}\stk{+}\myit{sizeof}(#1)}}
%\newcommand{\inchp}[1]{\ensuremath{\mem{:=}\mem{+}\myit{sizeof}(#1)}}
\newcommand{\incsk}[1]{\ensuremath{\myit{inc\_stk}(#1)}}
\newcommand{\inchp}[1]{\ensuremath{\myit{inc\_hp}(#1)}}
\newcommand{\decsk}[1]{\ensuremath{\myit{dec\_stk}(#1)}}
\newcommand{\dechp}[1]{\ensuremath{\myit{dec\_hp}(#1)}}
\newcommand{\cimplies}{\approx\!\!>}
%%%%%%%%%%%%%%%%
%\newcommand{\report}[1]{ }
%\newcommand{\paper}[1]{#1}
\newcommand{\acm}[1]{}
%%%%%%%%%%%%%%%%
\newcommand{\hide}[1]{}
\newcommand{\nil}{\btt{null}}
\newcommand{\cnil}{\btt{NULL}}
\newcommand{\res}{\btt{res}}
\newcommand{\ra}{\,\rightarrow\,}
\newcommand{\emp}{\btt{emp}}
\newcommand{\veq}{\ensuremath{\equiv}}
\newcommand{\self}{\btt{root}}
%\newcommand{\root}{\btt{root}}
\newcommand{\wwith}{\btt{inv}}
\newcommand{\equivimp}{\ensuremath{\Longleftrightarrow}}
\newcommand{\revimp}{\ensuremath{\Longleftarrow}}
\newcommand{\ndet}{\ensuremath{\wedge}}
\newcommand{\puret}{\ensuremath{\pi}}
%\newcommand{\simp}{\ensuremath{\textrm{--}\!\btt{*}}}
\newcommand{\simp}{{\bf ;}}
\newcommand{\minv}{\ensuremath{\iota}}
\newcommand{\ptr}{\ensuremath{\gamma}}
\newcommand{\nm}{\ensuremath{\phi}}
\newcommand{\heap}{\ensuremath{\kappa}}
\newcommand{\constr}{\ensuremath{\mathrm{\Phi}}}
\newcommand{\pconstr}{\ensuremath{\phi}}
\newcommand{\sat}[1]{\myit{SAT}(#1)}
\newcommand{\hmodels}[2]{\ensuremath{#1\,{\models}\,#2}}
\newcommand{\abduct}[2]{\ensuremath{#1 \rhd #2}}
\newcommand{\nabduct}[2]{\ensuremath{#1 \ntriangleright #2}}
\newcommand{\entail}[2]{\ensuremath{#1 \vdash #2}}
\newcommand{\entailA}[2]{\ensuremath{#1 \triangleright #2}}
\newcommand{\nentail}[2]{\ensuremath{#1 \nvdash #2}}
\newcommand{\entailD}[3]{\ensuremath{#1{\vdash}#2\,{\sep}\,#3}}
\newcommand{\entailH}[3]{\ensuremath{#1{\vdash}#2\,{\sep}\,#3}}
%\newcommand{\entailE}[4]{\ensuremath{#2{\vdash}#3\,{\sep}\,#4}}
\newcommand{\entailE}[4]{\ensuremath{#2{\vdash}_{#1}#3\,{\sep}\,#4}}
\newcommand{\entailV}[3]{\entailE{V}{#1}{#2}{#3}}
\newcommand{\entailK}[5]{\ensuremath{#3{\vdash}^{#1}_{#2}#4\,{\sep}\,#5}}
\newcommand{\entailVV}[3]{\entailK{\heap}{V}{#1}{#2}{#3}}
\newcommand{\entailI}[3]{\ensuremath{#2 \vdash_{#1} #3}}
\newcommand{\satisf}[3]{\ensuremath{(#1,#2) \vDash #3}}

\def\smstack{\myit{s}}
\def\smheap{\myit{h}}
\def\disjoint{\perp}

\newcommand{\myit}[1]{\textit{#1}}
\newcommand{\mytt}[1]{\texttt{#1}}
% \newcommand{\U}{\ensuremath{{\btt{U}}}}
\newcommand{\R}{\ensuremath{{\btt{R}}}}
\newcommand{\Le}{\ensuremath{{\btt{L}}}}
\newcommand{\Sh}{\ensuremath{{\btt{S}}}}
\newcommand{\A}{{\myit{A}}}
\newcommand{\at}{\mytt{@}}
\newcommand{\isview}{\myit{IsView}}
\newcommand{\isdata}{\myit{IsData}}
\newcommand{\hc}[2]{\ensuremath{{#1}{::}#2}}
\newcommand{\hx}[1]{\hc{\code{x}}{#1}}
\newcommand{\mtype}[2]{\ensuremath{{#1}{ \ :}#2}}
\newcommand{\stype}[2]{\ensuremath{{#1}{:}#2}}
\def\primeV{\myit{prime}}
\def\entword{ENT}
\newcommand{\rulen}[1]{\ensuremath{{\bf \scriptstyle #1}}}
\newcommand{\plainrule}[1]{[\underline{\ensuremath{{\bf \scriptstyle }\rulen{#1}}}]}
\newcommand{\entrule}[1]{\ensuremath{\scriptstyle \entword-#1}}
\newcommand{\entrulen}[1]{[\underline{{\bf \scriptstyle \entword-}\rulen{#1}}]}
\newcommand{\lemrulen}[1]{[{{\bf \scriptstyle LEM-}\rulen{#1}}]}
\newcommand{\lemnormrulen}[1]{\lemrulen{NORM-#1}}
\newcommand{\ebpentail}[2]{
	\begin{prooftree}
		\Hypo{\entrulen{#1}}
		\Infer[no rule]1{{\begin{prooftree}[rule style=simple] #2 \end{prooftree}}}
	\end{prooftree}
}
\newcommand{\entwlbl}[2]{{\begin{array}{c} { \entrulen{#1} } \\ {#2} \end{array} }}
%\newcommand{\entwlbl}[2]{{ { \entrulen{#1} } \\ {#2} }}
\newcommand{\verirulen}[1]{[\underline{{\bf \scriptstyle FV-}\rulen{#1}}]}
\newcommand{\reasonrulen}[1]{[\underline{{\bf \scriptstyle FR-}\rulen{#1}}]}
\newcommand{\ebpverif}[2]{
  \ifthenelse{\equal{#1}{} }{
    \begin{prooftree}[rule style=simple] #2 \end{prooftree}
   }{  
     \begin{prooftree}
       % \Hypo{\verirulen{#1}}
       \Hypo{[\underline{{\bf \scriptstyle }\rulen{#1}}]}
       \Infer[no rule]1{{\begin{prooftree}[rule style=simple] #2 \end{prooftree}}}
     \end{prooftree}
   }}
%
%\newcommand{\entail}[2]{\ensuremath{#1 \vdash #2}}
%\newcommand{\ebpverif}[2]{
	%\begin{prooftree}
		%\Hypo{\verirulen{#1}}
		%\Infer[no rule]1{ #2 }
	%\end{prooftree}
%}
%\newcommand{\hform}[3]{\ensuremath{{#1}{::}{#2}{\langle}{#3}{\rangle}}}
\newcommand{\hformn}[3]{\ensuremath{{\btt{#1}}{\mapsto}{\btt{#2}}{\langle}{\btt{#3}}{\rangle}}}
%\newcommand{\view}[2]{\ensuremath{#1{\langle}{#2}{\rangle}}}
%\newcommand{\hform}[3]{\ensuremath{{#2}{\langle}{#1,#3}{\rangle}}}
%\newcommand{\mapview}[3]{\ensuremath{{#1}{\mapsto}{#2}{\langle}{#3}{\rangle}}}
\newcommand{\view}[2]{\ensuremath{#1{(}{#2}{)}}}
\newcommand{\pview}[2]{\ensuremath{\overline{#1}{(}{#2}{)}}}
\newcommand{\sspec}[3]{\ensuremath{\view{\mathcal{#1}}{#2,#3}}}
\newcommand{\hform}[3]{\ensuremath{{#2}({#1,#3})}}
\newcommand{\uhform}[3]{\ensuremath{\code{H}({#2})({#1,#3})}}
\newcommand{\mapview}[3]{\ensuremath{{#1}{\mapsto}{#2}{(}{#3}{)}}}
\newcommand{\node}[3]{\hformn{#1}{#2}{#3}}
\newcommand{\transit}{\rightarrow}
\newcommand{\arrimp}{\ensremath{\,\btt{*}\!\!\!\rightarrow}\,}
% \newcommand{\state}[1]{\ensuremath{{\langle}#1{\rangle}}}
% \newcommand{\drule}[2]{\ensuremath{\frac{#1}{#2}}}
% \newcommand{\drulea}[2]{\ensuremath{\begin{array}{c}{#1}\\\hline{#2}\end{array}}}
% \newcommand{\dyn}[2]{\ensuremath{\state{#1}{\hookrightarrow}\state{#2}}}
% \newcommand{\dyns}[2]{\ensuremath{\state{#1}{\hookrightarrow^*}\state{#2}}}
% \newcommand{\dynf}[1]{\ensuremath{\state{#1}{\not\hookrightarrow^*}}}
% \newcommand{\dynerr}[1]{\ensuremath{\state{#1}{\hookrightarrow}{\err}}}
% \newcommand{\dynmemerr}[1]{\ensuremath{\state{#1}{\hookrightarrow}{\memerr}}}
% \newcommand{\dynothererr}[1]{\ensuremath{\state{#1}{\hookrightarrow}{\othererr}}}
\def\postst{\myit{Post}}


%used in heap constraint solving
\def\rewrite{\leadsto}
%\def\map{\myit{map}}
\def\map{\myit{X{\!}Pure}}
\def\mappair{\myit{X{\!}Pure}_P}
%\def\mapview{\ensuremath{\myit{X{\!}Pure}_V}}
\def\mapself{\myit{mapself}}
\def\mapi{\myit{mapI}}
%\def\mapviewi{\myit{mapvI}}
\def\mapselfi{\myit{mapsI}}
\def\findu{\myit{find}}
\def\fold{\myit{fold}_V}
\def\foldN{\myit{fold}}
\def\foldK{\myit{fold}^{\heap}}
\newcommand{\foldKI}[1]{\myit{fold}^{#1}}
\def\unfold{\myit{unfold}}
\def\alias{\myit{alias}}
\def\merge{\myit{merge}}
\def\overlap{\myit{overlap}}
\def\ex{{\bf ex}}

%def\M{\myit{M}}
%def\C{\myit{C}}
%def\I{\myit{I}}
%def\E{\myit{E}}
%def\A{\myit{A}}
%def\B{{\myit{B}}}
\def\D{\Delta}
%def\S{{\cal S}}
%def\H{{\cal H}}
%def\W{{\cal M}}
%\def\loop{\ensuremath{\alpha}}
\def\myloop{\ensuremath{\alpha}}
\def\arity{\myit{arity}}
\def\max{\myit{max}}
\def\fresh{\myit{fresh}}
\def\where{\btt{where}}
\def\bag{\ensuremath{\code{B}}}
\def\bagunion{\sqcup}
\def\bagintersect{\sqcap}
\def\bagsubsume {\sqsubset}
\def\bagsubtract{-}
\def\zerobag{\{{\bf 0}\}}
\newcommand{\load}[1]{\mytt{load}{\langle}#1{\rangle}}
\newcommand{\store}[1]{\mytt{store}{\langle}#1{\rangle}}
%\def\store{\mytt{store}}
\newcommand{\const}[1]{\mytt{const}{\langle}#1{\rangle}}
%\def\iconst{\mytt{iconst}}
\def\invoke{\mytt{invoke}}
\def\invokeTail{\mytt{invoke}_{Tail}}
\def\new{\mytt{new}}
\def\dispose{\mytt{dispose}}
\def\bool{\btt{bool}}
\def\int{\btt{int}}
\def\longint{\mytt{long}}
\def\float{\btt{float}}
\def\double{\mytt{double}}
\def\fixpt{\myit{fixpt}}
\def\rec{\mytt{Rec}}
\def\void{\btt{void}}
\def\type{\myit{type}}
\def\reference{\mytt{ref}}
\def\object{\mytt{object}}
\def\objectset{{\rm\bf ObjectType}}
\def\mn{\myit{m}}
\def\F{{\cal F}}%stack frame size
\def\phiinv{\phi_{\myit{inv}}}
\def\phirec{\phi_{\myit{rec}}}
\def\pre{\constr_{\myit{pr}}}
\def\post{\constr_{\myit{po}}}
\def\T{\Gamma}%type for the stack frame
\def\eqt{\myit{eq}_\tau}
%\def\stk{\pi} %current stack frame
\def\FS{\Pi}  %the stack of frames
\def\true{\btt{true}}
\def\false{\btt{false}}
%\def\a{\alpha}
\def\a{s}
\def\restrict{\myit{enrich}}%context enhance
\newcommand{\parg}[1]{\ensuremath{{\langle}#1{\rangle}}}
%% \newcommand{\hash}{\ensuremath{{\scriptstyle \#}}}
\newcommand{\num}[1]{|#1|}
\newcommand{\ifEq}[2]{\mytt{if}~#1~#2}
\newcommand{\whileEq}[1]{\mytt{while}~#1}
\newcommand{\myif}[3]{\btt{if}~(#1)~#2~\btt{else}~#3}
\newcommand{\mywhile}[3]{\btt{while}~#1~\btt{where}~#3~\btt{do}~#2}
\newcommand{\mybind}[3]{\mytt{bind}~#1~\mytt{to}~#2~\mytt{in}~#3}
\def\skipcmd{\mytt{nop}}
\newcommand{\defs}{\ensuremath{=_{df}}}
\newcommand{\snd}[1]{\myit{snd}(#1)}
\newcommand{\guarding}{{\ensuremath{\rightarrow}}}
\newcommand{\nonneg}[1]{\myit{notneg}(#1)}
\newcommand{\code}[1]{{\ensuremath{\tt #1}}}
\newcommand{\sm}[1]{\mbox{$#1$}}
\newcommand{\btt}[1]{{\tt #1}}
\newcommand{\todo}[1]{{\bf(* #1 *)}}
% \newcommand{\passref}{\btt{ref}}
\newcommand{\passref}[2]{#1{\footnotesize{\&}}~#2}
\newcommand{\ensures}{\btt{ensures}}
\newcommand{\requires}{\btt{requires}}

\newcommand{\llin}[1]{\texttt{#1}}

%%below renamed for llncs format
\newtheorem{thm}{Theorem}
%\newtheorem{lemma}{Lemma}
\newtheorem{pty}{Property}
%\newtheorem{cor}[thm]{Corollary}
\newtheorem{defn}{Definition}
\newtheorem{idfn}{Informal Definition}
\def\proof{\vspace{-0.2cm}\noindent{\bf Proof}\hspace*{0.5cm}}
%\newcommand{\tverb}[1]{\mbox{\verb|#1|}}

%\newcommand{\tcv}[2]{#1\,\vdash\,#2}
\newcommand{\tcv}[3]{#1\,\vdash\,#2,\,#3}
\newcommand{\tcvT}[2]{\tcv{}{#1}{#2}}


%frame bound inference
\newcommand{\fsr}[5]{#1 \vdash_{\small\myit{F}} #2 \rightsquigarrow #3, #4, #5}
\newcommand{\fsinf}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{FS-#1}}]\\[0.5ex]
#2\end{array}}{#3}}}
%\newcommand{\rulen}[1]{\ensuremath{{\bf \scriptstyle #1}}}

%abstract state inference
\newcommand{\asr}[4]{#1 \vdash_{\small\myit{A}} #2 \rightsquigarrow #3, #4}
\newcommand{\asinf}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{AS-#1}}]\\[0.5ex]
#2\end{array}}{#3}}}

%stack space inference
\newcommand{\ssrA}[2]{\ssr{\myit{a}}{#1}{#2}}
\newcommand{\ssr}[3]{#1 \vdash_{\small\myit{S}} #2 \rightsquigarrow #3}
\newcommand{\ssinf}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{SS-#1}}]\\[0.5ex]
#2\end{array}}{#3}}}

%heap space inference
\newcommand{\hsrX}[5]{#5,#1 \vdash_{\myit{H}} #2 \rightsquigarrow #3,#4}
\newcommand{\hsr}[4]{\hsrX{#1}{#2}{#3}{#4}{\myit{a}}}
%\newcommand{\hsr}[4]{\myit{a},#1 \vdash_{\myit{H}} #2 \rightsquigarrow #3,#4}
\newcommand{\hsinf}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{HS-#1}}]\\[0.5ex]
#2\end{array}}{#3}}}

%op semantics
\newcommand{\oprerr}[5]{\ensuremath{\config{#1}{#2}{#3}{#4}\hookrightarrow #5}}
%\newcommand{\config}[4]{\ensuremath{{\langle}{#1},{#2},{#3},{#4}{\rangle}}}
%\newcommand{\opr}[8]{\ensuremath{\config{#1}{#2}{#3}{#4} \hookrightarrow \config{#5}{#6}{#7}{#8}}}
%\newcommand{\oprd}[4]{\opr{\FS}{#1}{\O}{#2}{\FS}{#3}{\O}{#4}}
\newcommand{\config}[4]{\ensuremath{{\langle}{#1},{#2},{#3},{#4}{\rangle}}}
\newcommand{\opr}[8]{\ensuremath{\config{#1}{#2}{#3}{#4} \hookrightarrow \config{#5}{#6}{#7}{#8}}}
\newcommand{\oprd}[4]{\opr{#1:\FS}{\O}{#2}{\ss,\mem}{#3:\FS}{\O}{#4}{\ss,\mem}}
\newcommand{\oprds}[6]{\opr{#1:\FS}{\O}{#2}{\ss,\mem}{#3:\FS}{#4}{#6}{\ss,#5}}
\newcommand{\oprc}[5]{\config{#1}{#2}{#3}{#4}\hookrightarrow^* {#5}}
\newcommand{\oprule}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{OP-#1}}]\\[0.5ex]
#2\end{array}}{#3}}}

\def\EI{\epsilon}
\def\Y{\Upsilon}
\def\L{\Lambda}
\def\O{\omega}
\def\i{\iota}
%\def\mem{\mytt{h}}%available heap space
%\def\ss{\mytt{s}}%available stack space
\def\MemErr{\mytt{MemInadequate}}
\def\OF{\mytt{FrameErr}}
\def\cf{\myit{f}}
\def\ret{\mytt{ret}}
\def\size{\myit{size}}
\def\cxt{\mytt{cxt}}
\newcommand\reqs[4]{\ensuremath{#1 \vdash #2 \rightsquigarrow #3,#4 }}

\def\G{\Gamma}
%\def\res{\myit{res}}
%\def\nochange{\myit{no}\!{\cal X}}
\def\nochange{\myit{nochange}}
\def\FSV{\myit{V}}
\newcommand{\sep}{\ensuremath{*}}
\newcommand{\sepc}{\ensuremath{*}}
\newcommand{\rview}[2]{\code{\ensuremath{#1{(}{\self,#2}{)}}}}
\newcommand{\sepimpl}{\ensuremath{\code{-\!\!\!\!-\!\!\!*}}}
\newcommand\eq[3]{\ensuremath{\myit{eq}_{#1}(#2,#3)}}
\newcommand{\tj}[5]{#1,#2\,{\vdash}\,#3~{::}~#4, #5}
%\newcommand{\tr}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{S-#1}}]\\[0.5ex]
%#2\end{array}}{#3}}}
\newcommand{\tr}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{#1}}]\\[0.5ex]
#2\end{array}}{#3}}}
\newcommand{\hlr}[3]{\ensuremath{\frac{\begin{array}{c}\reasonrulen{#1}\\[0.5ex]%[\underline{\rulen{#1}}]\\[0.5ex]
#2\end{array}}{#3}}}
\newcommand{\hlrs}[3]{\ensuremath{\frac{\begin{array}{c}%\verirulen{#1}\\[0.5ex]%[\underline{\rulen{#1}}]\\[0.5ex]
#2\end{array}}{#3}}}
\newcommand{\htriple}[3]{\ensuremath{\vdash \{#1\}\,{\color{blue}{#2}}\,\{#3\}}}
%\newcommand{\rulen}[1]{\ensuremath{{\bf \scriptstyle #1}}}
\newcommand{\iview}[2]{\ensuremath{#1{\langle}#2{\rangle}}} %use it rather than tt
\newcommand{\ihc}[2]{\ensuremath{#1{::}#2}}                 %use it rather than tt
\newcommand{\subtr}[3]{\entailH{#1}{#2}{#3}}
%\newcommand{\subtr}[3]{\ensuremath{#1\,{\vdash}\,#2,#3}}
\newcommand{\reasonrulenm}[1]{[\underline{{\bf \scriptstyle }\rulen{#1}}]}
\newcommand{\hlrm}[3]{\ensuremath{\frac{\begin{array}{c}\reasonrulenm{#1}\\[0.5ex]%[\underline{\rulen{#1}}]\\[0.5ex]
#2\end{array}}{#3}}}

%static semantics
\newcommand{\raws}[9]{{#1} ; {#2} ; {#3} ;{#4} \vdash {#5} :: {#6} , {#7},{#8} ,{#9}}
\newcommand{\rawss}[5]{\T ; \D; \L; \Y  \vdash {#1} :: {#2} , {#3}, {#4}, {#5}}

%from sound-cav.tex
\newcommand{\mymodel}{\models}
\def\Flds{\myit{Fields}}
\def\Store{\myit{Heaps}}
\def\Stack{\myit{Stacks}}
\def\Locations{\myit{Loc}}
\def\Val{\myit{Val}}
\def\Var{\myit{Var}}
\newcommand{\mo}[3]{#1,#2 \mymodel #3}
\newcommand{\notmo}[3]{#1,#2 \not\mymodel #3}
\newcommand{\mos}[1]{\ensuremath{\mo{s}{h}{#1}}}
\newcommand{\mosp}[1]{\ensuremath{{s}\mymodel{#1}}}
\def\iffs{\mbox{\tt iff~}}
\def\dom{\myit{dom}}
\def\loc{\iota}
\newcommand{\s}[1]{[\![#1]\!]s}
\def\inv{\myit{inv}}
\def\getP{\myit{getProperty}}
\newcommand{\menv}[2]{\frac{\begin{array}{c}#1\end{array}}{#2}}
\def\fresh{\myit{fresh}}
\def\length{\myit{length}}

\newcommand{\mysf}[1]{\textsf{\bf\small #1}}
% \newcommand{\Top}{\mbox{$\top$}}
\newcommand{\presize}{\phi_{\myit{pr}}}
\newcommand{\postsize}{\phi_{\myit{po}}}
\newcommand{\sizev}{{\cal V}}
\newcommand{\pure}{\ensuremath{\pi}}
\newcommand{\sarg}[1]{{\la}#1{\ra}}
\def\la{\langle}
\def\ra{\rangle}
%\def\bag{B}
\def\bagconstr{\varphi}

\newcommand{\pnt}[2]{\ensuremath{#1 {\mapsto} #2}}
\newcommand{\lseg}[2]{\ensuremath{\mathsf{ls}(#1, #2)}}
\newcommand{\lsegs}[3]{\ensuremath{\mathsf{ls}(#1, #2, #3)}}


\newcommand{\hipsleek}{\textsc{Hip/Sleek}~}
\newcommand{\hip}{\textsc{Hip}~}
\newcommand{\sleek}{\textsc{Sleek}~}
\newcommand{\M}{\mathsf{M}}

\newcommand{\absr}[3]{\ensuremath{\frac{\displaystyle{#1}}
    {\displaystyle{#2}}{\textsc{#3}}}}

\newcommand{\join}[2]{\ensuremath{\msf{join}(#1,#2)}}
\newcommand{\pjoin}[2]{\ensuremath{\msf{join_\pure}(#1,#2)}}
\newcommand{\ljoin}[2]{\ensuremath{\lift{\msf{join}}(#1,#2)}}
\newcommand{\widen}[2]{\ensuremath{\msf{widen}(#1,#2)}}
\newcommand{\pwiden}[2]{\ensuremath{\msf{widen_\pure}(#1,#2)}}
\newcommand{\lwiden}[2]{\ensuremath{\lift{\msf{widen}}(#1,#2)}}
\newcommand{\joining}{\ensuremath{\msf{join}}}
\newcommand{\widening}{\ensuremath{\msf{widen}}}
%\newcommand{\abs}{\leadsto}
\newcommand{\cfm}{\Lambda}
\newcommand{\junk}{\textit{junk}}

%%%%%%

\def\hip{\textsc{Hip}~}
\def\sleek{\textsc{Sleek}~}
\def\Prog{\ensuremath{\mathcal{P}}}
\def\shps{\ensuremath{\mathcal{S}}}
\def\fail{\textsf{fail}}
\def\entfailed{\myit{entfail}}
\newcommand{\numerical}[1]{\ensuremath{\mathsf{pureV}(#1)}}
\newcommand{\abstraction}[1]{\ensuremath{\mathsf{gen\_abs}(#1)}}
\newcommand{\postprime}[1]{\ensuremath{\mathsf{prime}(#1)}}
\newcommand{\Reach}[2]{\ensuremath{\mathsf{Reach}(#1, \{#2\})}}
\newcommand{\Local}[2]{\ensuremath{\mathsf{Local}(#1, \{#2\})}}
\newcommand{\Frame}[2]{\ensuremath{\mathsf{Frame}(#1, \{#2\})}}
\newcommand{\pr}[1]{\ensuremath{\mathsf{ex\_quan}(#1)}}
\newcommand{\pureres}[1]{\code{#1}}
\def\Sp{\Prog}
\newcommand{\lbl}[1]{\ensuremath{\myit{lbl}(#1)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{ language=[ANSI]C,
  basicstyle=\ttfamily\small,
  keywordstyle=\color{black}\ttfamily,
  % keywordstyle=\color{blue},
  % numbers=left,
  % numberstyle=\scriptsize,
  % stepnumber=1,
  % numbersep=5pt,
  commentstyle=\small\color{red},
  % backgroundcolor=\color[rgb]{0.9,1.0,1.0},
  % frame=single,
  framexleftmargin=0mm,
  xleftmargin=0mm,
  xrightmargin=0mm,
  % resetmargins=true,
  % rulesepcolor=\color{red!20!green!20!blue!20!},
  captionpos=b, 
  showspaces=false,
  showstringspaces=false,   
  showtabs=false, 
  tabsize=4,
  breaklines=true,
  % lineskip=0pt;
  extendedchars=false,
  % morekeywords={self,requires,ensures,data},
  escapeinside= {(*@} {@*)}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%space def

\newcommand{\dist}{0em}
\newcommand{\distv}{0em}
\newcommand{\disth}{0em}
\newcommand{\distt}{0em}

\newcommand{\distf}{-1.6ex}

% \newcommand{\sstate}[1]{\textcolor{MidnightBlue}{\code{#1}}}
\newcommand{\obar}[1]{\code{\bar{#1}}}

\newcommand{\viewbody}{\L}
% \newcommand{\prot}{\myit{G}}
\newcommand{\prot}{{G}}
\newcommand{\prott}{\ensuremath{\prot^\mathcal{T}}}
\newcommand{\proj}{{L}}
\newcommand{\projp}{\Upsilon}
\newcommand{\projc}{\proj}
\newcommand{\unkbox}{\square}
\newcommand{\sessend}{end}

\newcommand{\send}[2]{
  \ifthenelse{\equal{#1}{} }{
     !{#2}
   }{  !{#1}{\cd}{#2}}
 }
\newcommand{\recv}[2]{
   \ifthenelse{\equal{#1}{} }{
     ?{#2}
   }{  ?{#1}{\cd}{#2}}
 }
\newcommand{\sendc}[3]{
  \ifthenelse{\equal{#2}{} }{
     #1!{#3}
  }{ #1!{#2}{\cd}{#3} }
}
\newcommand{\recvc}[3]{
  \ifthenelse{\equal{#2}{} }{
     #1?{#3}
  }{ #1?{#2}{\cd}{#3} }
}
  
\newcommand{\trans}[2]{\unkbox {#1}{\cd}{#2}}

\newcommand{\seq}{;} %sequence
\newcommand{\cpar}{\|} %parallel composition
%\newcommand{\useq}{*} %order insensitive conj
% \newcommand{\useq}{\circledast}
\newcommand{\useq}{*}
\newcommand{\disj}{\vee}
\newcommand{\chan}{\mathcal{C}}
\newcommand{\lchan}{{\mathcal{C}}}
\newcommand{\chani}[3]{\ensuremath{\view{\chan}{#1,#2,#3}}}
\newcommand{\lchani}[3]{\ensuremath{\view{\lchan}{#1,#2,#3}}}
\newcommand{\chant}[2]{\ensuremath{\view{\chan}{#1,#2}}}
%second order variable
%second order variable for heap formula
%second order variable for session
\newcommand{\hov}{V}
\newcommand{\hovars}{\hov}
\newcommand{\hovarh}{\hov}
\newcommand{\hosets}{\mathcal{I}}
\newcommand{\hoseth}{\mathcal{I}}
\newcommand{\vdashs}{\vdash_{s}}
\newcommand{\vdashe}{\vdash_{e}}
\newcommand{\entailS}[3]{\ensuremath{#1 \vdash #2 ~\leadsto ~#3}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SYNC related stuff (fence,cdl, etc)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\gfencelit{f}
\def\genfencelit{F}
\def\pfencelit{{f}}
\def\sync{\ensuremath{\zeta}}
\def\await{await}
\def\down{down}
\def\cons{}
\def\acc{+}

%\newcommand{\fence}[3]{
%\ifthenelse{\equal{#1}{-} }{
  %{#3}^\bullet({#2})
%}{
  %\ifthenelse{\equal{#1}{+} }{
		%{#3}^\circ({#2})
%}{
		%{#3}^\circ({#2},#1)
%}}}
\newcommand{\fence}[4]{
\ifthenelse{\equal{#1}{-} }{
  {#4}^\text{\cons}({#2},#3)
}{\ifthenelse{\equal{#1}{+} }{
{#4}^\text{\acc}({#2},#3)
}{\ifthenelse{\equal{#1}{D} }{
{\down}^\text{\acc}({#2},#3)
}{\ifthenelse{\equal{#1}{A} }{
{\await}^\text{\cons}({#2},#3)
}{{\sync}^\text{}({#2})} } 
}}}

%\newcommand{\gensync}[1]{}

%%%%% global fence
\def\gfenceboth{\rightleftharpoons}
\def\gfencesend{\leftharpoonup}
\def\gfencereceive{\rightharpoondown}
\newcommand{\ggfence}[3]{\fence{#1}{#2}{#3}{\gfencelit}}
\newcommand{\gstub}[3]{\fence{#1}{#2}{#3}{\gfencelit}}
\newcommand{\gfence}[4]{
\ifthenelse{\equal{1}{#3} }{
#1{\gfencereceive}#2:#4 % fencing on the receiver
}{
\ifthenelse{\equal{2}{#3} }{
#1{\gfencesend}#2:#4   % fencing on the sender
}{
#1{\gfenceboth}#2:#4   % unknown source for fencing
}}}
\newcommand{\pfence}[3]{\fence{#1}{#2}{#3}{\pfencelit}}
\newcommand{\fences}{\mathcal{F}}
\newcommand{\stripfence}[1]{\ensuremath{#1\%\sync}}
\newcommand{\opt}[1]{[#1]}

\newcommand{\upeergfence}[2]{\ensuremath{\gfence{\unkbox}{\unkbox}{#1}{#2}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PROJECTION related stuff 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\projectsymbol}{\downharpoonright}
\newcommand{\project}[2]{(#2){\projectsymbol}_{#1}}

\newcommand{\bind}[2]{#1~$\leftarrow$~#2}
\newcommand{\mapschan}[2]{\ensuremath{#1\vDash#2}}

\def\pequiv{\dashv\vdash}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MISC 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{projcolor}{RGB}{0, 176, 80} %green
\definecolor{protcolor}{RGB}{222, 71, 142} %pink
\definecolor{fencecolor}{RGB}{0, 176, 240} %blue

\newcommand{\setfont}[2]{{\fontfamily{#1}\selectfont #2}}

\newcommand{\savespace}{\vspace{-2mm}}
\def\dual{\ensuremath{\sim}}
\def\resid{S}
\def\chanvar{c}
\def\lchanvar{{c_1}}
\def\rolevar{P}
\def\employ{\in}
\def\notemploy{\notin}
\def\eqdef{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny
          def}}}{=}}}

\newcommand\figref[1]{Fig. \ref{#1}}
\newcommand\defref[1]{Def. \ref{#1}}
\newcommand\axiomref[1]{Axiom \ref{#1}}
\newcommand\secref[1]{Sec. \ref{#1}}
\newcommand\chapref[1]{Chapter \ref{#1}}

% roman god of communication 
\def\sessionlogic{Mercurius}

\newcommand{\excerpt}[1]{\parbox[t]{\textwidth}{\raggedleft\parbox[c]{.85\textwidth}{
      \linespacing{1.25} 
      \raggedleft
      #1
      \vspace{4ex}}}}


\newtheorem{theorem}{Theorem}
\newtheorem*{remark}{Remark}
\newtheorem{axiom}{Axiom}
\renewenvironment{proof}{\noindent{\bf Proof:}}{\qedsymbol}

% \newcommand{\racefreerel}[2]{\ensuremath{#1 \circ #2}}
\newcommand{\racefreerel}[2]{{\ifthenelse{\equal{#2}{}}{RF(#1)}{RF(#1,#2)}}}
\def\wrt{w.r.t.~}
\def\ifonlyoif{\ensuremath{\Leftrightarrow}}
\def\imply{\ensuremath{\Rightarrow}}
\def\pspace{\\~\\}
\newcommand{\adjacent}[2]{\text{\textbardbl} #1\seq#2
  \text{\textbardbl}}

\newcommand{\graph}[1]{
  \ifthenelse{\equal{#1}{}}{\mathcal{G}}{\mathcal{G}^#1}}
\def\contraction{\xi}
\newcommand{\contract}[2]{\contraction(#1,#2)}
\newcommand{\ccontract}[3]{\overline{\contraction}(#1,#2)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% global protocol related stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\explicitseq}[1]{
  \ifthenelse{\equal{RR}{#1} }{
    {\downdownharpoons} %% \downdownarrows
  }{
    \ifthenelse{\equal{SS}{#1} }{
      \upupharpoons %% \upuparrows
    }{
      \ifthenelse{\equal{RS}{#1} }{
        \downupharpoons %% \downuparrows
      }{
        \ifthenelse{\equal{SR}{#1} }{
          \updownharpoons%% \updownarrows
        }{

        }         
      }   
    }
  }
}

\newcommand{\gseq}[1]{\ensuremath{\seq^{\explicitseq{#1}}}}
\newcommand{\gseqA}[1]{\ensuremath{\seq}}
\newcommand{\guard}[1]{\ensuremath{{\ominus}(#1)}}
\newcommand{\assume}[1]{\ensuremath{{\oplus}(#1)}}
%% \newcommand{\assumeL}[2]{\ensuremath{\oplus(#1)_{#2}}}
\newcommand{\assumeL}[2]{\ensuremath{\oplus(#1)}}

%% A->B : k <\delta>  where
%% #1 --> A
%% #2 --> B
%% #3 --> \delta
%% #4 --> k
%% #5 --> transmit ->, labelled or not
\newcommand{\transmitbase}[5]{
  \ifthenelse{\equal{#3}{} \AND \equal{#4}{}}{
    #1{#5}#2
  }{
    \ifthenelse{\NOT \equal{#3}{} \AND \equal{#4}{}}{
      #1{#5}#2:#3
    }{
      \ifthenelse{\NOT \equal{#4}{} \AND \equal{#3}{}}{
        #1{#5}#2:#4
      }{
        #1{#5}#2:#4{\langle}#3{\rangle}
      }
    }
  }
}

\newcommand{\transmit}[4]{\transmitbase{#1}{#2}{#3}{#4}{\rightarrow} }
\newcommand{\delegate}[3]{\transmitbase{#1}{#2}{#3}{}{\xrightarrow{d}}
}
\newcommand{\atransmit}[5]{\transmitbase{#1}{#2}{#3}{#4}{\xrightarrow{#5}}}
\newcommand{\msg}[2]{#1\,{\cdot}\,#2}
\newcommand{\omsg}[2]{#2}

\newcommand{\peer}[1]{Peer(#1)}
\newcommand{\bindv}[2]{Bind(#1,#2)}
 
\def\inact{\emp}
\newcommand{\zoom}[2]{#1\%#2}
\newcommand{\last}[2]{last(#1,#2)}
\newcommand{\first}[2]{first(#1,#2)}
%% delegation

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CDL related stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% global CDL
\newcommand{\gdown}[3]{#1:#2 {\langle} DOWN(#3) {\rangle}}
\newcommand{\gawait}[3]{#1:#2 {\langle} AWAIT(#3) {\rangle}}
% local CDL
\newcommand{\pdown}[1]{down(#1)}
\newcommand{\pawait}[1]{await(#1)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% causality related stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\atid{\textit i}
\def\atloc{\textit l}
\def\atzero{\bot}

\def\implies{\Rightarrow}

\newcommand{\addL}[1]{\ensuremath{(#1,0)}}
\newcommand{\addR}[1]{\ensuremath{(0,#1)}}
\newcommand{\addFull}[0]{\ensuremath{1}}
\newcommand{\addAt}[1]{\ensuremath{{\at}#1}}
\def\atFull{\addAt{\addFull}}
\def\atL{\addAt{\addL{\addFull}}}
\def\atR{\addAt{\addR{\addFull}}}
\def\atLno{\addL{\addFull}}
\def\atRno{\addR{\addFull}}
\def\atLL{\addAt{\addL{\atLno}}}
\def\atLR{\addAt{\addL{\atRno}}}
\def\atRL{\addAt{\addR{\atLno}}}
\def\atRR{\addAt{\addR{\atRno}}}

\newcommand{\precx}[1]{\ensuremath{\prec_{#1}}}
\newcommand{\lt}[2]{#1\,{\prec}\,#2}
% \newcommand{\ltset}[2]{#1\,{\prec^*}\,#2}
\newcommand{\ltset}[2]{merge(#1,\,#2)}
\newcommand{\ltcb}[2]{#1{\prec_{CB}}\,#2}
\newcommand{\lthb}[2]{#1{\prec_{HB}}\,#2}
\newcommand{\lthbmay}[2]{#1{\prec^{maybe}_{HB}}\,#2}
% \newcommand{\rl}[2]{#1^{(#2)}}
% same as event
\newcommand{\rl}[2]{\event{#1}{#2}}
% \newcommand{\rrl}[3]{(#1,#2)^{(#3)}}
\newcommand{\rrl}[3]{\atransmit{#1}{#2}{}{}{#3}}
\newcommand{\rk}[3]{\rl{#1}{#3}{:}{#2}}
\def\roles{\mathcal{R}}

\def\oplusseq{\otimes}
\def\oplusstar{\circledast}
\def\opluschoice{\oplus}

\def\roletyp{\mathcal{R}{{ole}}}
\def\labeltyp{{{Nat}}}
\def\idtyp{nat}
\def\chantyp{\mathcal{C}{{han}}}
%% \def\chantyp{\Var}
\def\operationtyp{\mathcal{O}}

\def\ordering{\pure}
\newcommand{\chanmap}{\ensuremath{\mathrm{\Gamma}}}
\def\rolemap{K}
\def\locof{\mathcal{L}}
\def\loccompstar{\useq}
\def\loccompseq{\seq}
\def\loccompvee{\vee}
% \def\loccompstar{\bowtie}
% \def\loccompseq{\ltimes}
% \def\loccompvee{\vee}

\newcommand{\composeseq}[2]{{f_1}(#1,#2)}
\newcommand{\composestar}[2]{{f_2}(#1,#2)}
\newcommand{\composevee}[2]{{f_3}(#1,#2)}

\def\bordermergebase{\sqcup}
% \newcommand{\bordermerge}[1]{\bordermergebase^{#1}}
\newcommand{\bordermerge}[1]{\lfloor{#1}\rfloor}
\newcommand{\mergeseq}{\bordermerge{\loccompseq}}
\newcommand{\mergestar}{\bordermerge{\loccompstar}}
\newcommand{\mergevee}{\bordermerge{\loccompvee}}

\newcommand{\mergeseqtier}[2]{merge\_set(#1,#2)}
\newcommand{\mergestartier}[2]{merge\_star(#1,#2)}

% frontier
\def\mfront{F}
% backtier
\def\mback{B}
% constraints
\newcommand{\morders}{\ensuremath{\mathrm{\Pi}}}
% obligations
\def\mguards{S^{\ominus}}
\def\massum{S^{\oplus}}
\def\terminal{T}
\def\operation{E}
\newcommand{\notop}[1]{\neg(#1)}
\def\orderas{\vartheta}
\def\racefreeas{\ensuremath{\mathrm{\Psi}}}

\newcommand{\racefree}[2]{\ensuremath{#1 \,{\vDash}\,  #2}}
% constraint base formula
\def\cbformula{BForm}
% constraint formula
\def\cformula{EForm}
\def\eborder{\beta}
\def\tborder{\eborder^T}
\def\oborder{\eborder^E}


\definecolor{navyblue}{HTML}{336699}
\definecolor{denimblue}{HTML}{151B8D}
\newcommand\blueord[1]{\textcolor{denimblue}{#1}}
\newcommand\grayord[1]{\textcolor{gray}{#1}}

\def\fmsg{\St}
\newcommand\chanspec[3]{\chani{#1}{#2}{#3}}


\newcommand{\sstate}[1]{\textcolor{denimblue}{\textit{\code{#1}}}}
\newcommand{\lineno}[1]{\ensuremath{_{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%% listing style %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\commentcolor{purple!40!black}
\newcommand{\codecomment}[1]{\color{\commentcolor}{#1}}

\lstdefinestyle{customc}{
  belowcaptionskip=1\baselineskip,
  breaklines=true,
  % frame=L,
  % xleftmargin=\parindent,
  language=C,
  numbers=left,
  showstringspaces=false,
  basicstyle=\footnotesize\ttfamily,
  keywordstyle=\bfseries\color{green!40!black},
  % commentstyle=\itshape\color{purple!40!black},
  commentstyle=\itshape\color{\commentcolor},
  % identifierstyle=\color{blue},
  identifierstyle=\color{black},
  stringstyle=\color{orange},
}

\lstset{escapechar=@,style=customc}


